Inferring Mood-While-Eating with Smartphone Sensing and Community-Based Model Personalization

The interplay between mood and eating episodes has been extensively researched, revealing a connection between the two. Previous studies have relied on questionnaires and mobile phone self-reports to investigate the relationship between mood and eating. However, current literature exhibits several limitations: a lack of investigation into the generalization of mood inference models trained with data from various everyday life situations to specific contexts like eating; an absence of studies using sensor data to explore the intersection of mood and eating; and inadequate examination of model personalization techniques within limited label settings, a common challenge in mood inference (i.e., far fewer negative mood reports compared to positive or neutral reports). In this study, we sought to examine everyday eating behavior and mood using two datasets of college students in Mexico (N_mex = 84, 1843 mood-while-eating reports) and eight countries (N_mul = 678, 24K mood-while-eating reports), which contain both passive smartphone sensing and self-report data. Our results indicate that generic mood inference models experience a decline in performance in specific contexts, such as during eating, highlighting the issue of sub-context shifts in mobile sensing. Moreover, we discovered that population-level (non-personalized) and hybrid (partially personalized) modeling techniques fall short in the commonly used three-class mood inference task (positive, neutral, negative). To overcome these limitations, we implemented a novel community-based personalization approach. Our findings demonstrate that mood-while-eating can be inferred with accuracies 63.8% (with F1-score of 62.5) for the MEX dataset and 88.3% (with F1-score of 85.7) with the MUL dataset using community-based models, surpassing those achieved with traditional methods.

==> 04-Method.tex <==
\section{Methods}\label{sec:methods_of_rqs}


In this section, we discuss the experimental setup for the inference of mood while eating. The inference was carried out using several model types such as Random Forest (RF), Naive Bayes (NB), Support Vector Classification (SVC), XGBoost (XGB), and AdaBoost (AB) \cite{rf_inbook, rish2001empirical, natekin2013gradient, chen2016xgboost, schapire2013explaining, noble2006support}. These models were chosen by considering the characteristics of the dataset, such as the size, tabular nature, and interpretability. We used the Synthetic Minority Over-sampling Technique (SMOTE) \cite{chawla2002smote} for training sets and down-sampled testing sets to obtain balanced datasets for testing, hence having a baseline accuracy of 33.3\% for all experiments. Hyperparameter tuning was done with GridSearch. We used scikit-learn \cite{pedregosa2011scikit} along with python to carry out the experiments.

The three target classes of the experiment are: negative, neutral, and positive. We made inferences using many models, with different techniques for different degrees of personalization, to obtain a clear understanding of how the inference accuracy for mood inferences during eating episodes can be improved. The study was carried out using the following three approaches. 


\begin{itemize}[wide, labelwidth=!, labelindent=0 pt]
    \item \textbf{Population-Level Model (PLM):} We followed a population-level, leave-one-user-out strategy \cite{servia2017mobile, meegahapola2023generalization}. This approach involved utilizing the data of each target user as the testing set, while the remaining dataset was utilized for training the model. The objective of this strategy was to simulate a scenario in which models were created using data collected from a population utilizing a mobile health (mHealth) application with mobile sensing, and to evaluate the performance of these models on a new target user. Therefore, for each selected user, the model was trained using data from the remaining participants and then tested using the data of the target user. To enhance the robustness of the training process, for each target user, a randomly sampled subset of data from the population (90\%) was utilized for training, and a 30\% random sample of the target user's data was used for testing. This process was repeated five times for each user, and the results were subsequently averaged across all users.
    
    \item \textbf{Hybrid Model (HM):} This case is somewhat similar to PLM, but with a percentage of data from the target user included in the training set, which leads to a partially personalized model for that target user \cite{likamwa2013moodscope, meegahapola2023generalization}. The technique illustrates a model where the user has already used the sensing app for some time, and the model has been already personalized to some degree after getting some ground truth data via self-reports from the target user. In the testing phase, new data gathered from the same user will be used in the testing set. When conducting experiments, for each target user, the model training was done using 70\% of that user's randomly sampled data and a randomly sampled portion of data from other users (90\%) combined, and the rest of the data of that target user (30\%) was used to test the model. The process was iterated five times for each user. Finally, the results across all users were averaged.
    
    \item \textbf{Community-Based Model (CBM):} community-Based model is based on the similarity-based technique proposed in Section~\ref{subsec:method_rq3}, where for each target user, we extracted the community of that user empirically. To detect the community, different $th$ values were used, and different communities were tested for each user to find the best community. The training split was created using a randomly sampled set of data from the community of that user (90\%), together with 70\% of the target user's data. Then, the model was tested using the remaining 30\% of the data of the target user. The process was iterated five times for each user. Finally, the results across all users were averaged. 
    
\end{itemize}{}


We conducted experiments for all three approaches, using all the passive sensing features given in Table~\ref{table:allfeatures} for MEX and Table~\ref{table:allfeatures_dataset2} for MUL, that we obtained in the original datasets. These features have been inspired by prior studies \cite{meegahapola2021one, Biel2018, Meegahapola2020Alone, Meegahapola2021Survey}, and more details on how features were extracted are given in \cite{meegahapola2021one} and \cite{meegahapola2023generalization}.






\subsection{{RQ1: Generic Models and Context-specific Models Analysis}}\label{subsec:method_rq1}

In order to assess the performance of a generic mood inference model within specific contexts, we utilized the Multi-Country dataset (MUL) which provided information on the concurrent activities being performed by the participants at the time of self-reporting their mood. This dataset included a list of 12 broad activities, such as resting, walking, sports, eating, drinking, studying, and working. By utilizing this dataset, we were able to examine the performance of the mood inference model in different situated contexts, as the participants were engaged in various activities. This allows for an examination of the model's performance across a diverse range of settings.

First, we trained a mood inference model using the population-level approach on the MUL dataset. Then, we obtained a breakdown of the mood inference performance for the testing test, for each activity performed by users during the mood report. By examining the mood inference performance across different activities, we aimed to determine whether generic, one-size-fits-all models for mood inference are similarly effective across all situated contexts and whether context-specific models are necessary for eating behavior, as previously studied in the workplace context. Experiments were carried out in both population-level and hybrid modeling approaches, hence examining the partial personalization effect. Experiments were done five times with random sampling, and the results were averaged. Second, considering the total dataset of the size 329K mood reports including the 24K mood-while-eating reports, we conducted an analysis in which we kept the number of training data points from all the activities constant (280K mood reports) and increased the number of mood-while-eating reports in training set from 0 to 15000 (in steps 0, 2500, 5000, 7500, 10000, 12500, 15000). The testing set contained around 20K mood reports captured during other contexts and 2000 mood-while-eating reports. For each step, experiments were done five times with random sampling for training and testing sets, and the results were averaged. Hence, by increasing the number of mood-while-eating reports in the training set and observing the performance of the overall testing set, and in addition, to the 2000 mood-while-eating reports, we examined how the inclusion of data from a specific context affects model performance. Finally, while we reported results for this setup in later sections (considering page limitations and brevity), we also experimented with other different setups, as in, changing the size of the other mood reports in training (e.g., 100K, 150K, 200K, 250K instead of 280K, which is the maximum number of data points we could use for training) and testing sets (e.g., 2.5K, 5K, 10K, 15K instead of 20K, which is closer to the maximum number of data points we could use for testing), which did not yield contrasting conclusions or results. 




\subsection{{RQ2: Mood-While-Eating Inference}}\label{subsec:method_rq2}

For this section, we used both datasets. In MEX, we used the whole dataset as all mood reports corresponded to eating episodes, hence providing the mood-while-eating. However, in MUL, since there are over 329K mood reports, out of which a majority corresponded to different activities, we only used mood reports corresponding to eating episodes to examine this research question. We first trained population-level models and hybrid models to examine the effectiveness of mood inference. We conducted experiments with both approaches with multiple model types (RF, NB, SVC, XGB, AB) across both datasets. Then, we also discuss the reasons for not being able to examine and train user-level models for mood-while-eating inference in limited data settings from each individual. Hence here, we identify the need for a better personalization strategy for limited data setting. 














\subsection{{RQ3: Community-Based Model Personalization Approach}}\label{subsec:method_rq3}

\begin{figure*}[t]
\begin{center}
    \begin{minipage}[t]{\textwidth}
        \centering
        \includegraphics[width=0.75\textwidth]{images/mood-while-eating-architecture.png}
        \caption{High-Level Architectural View of the Community-based Personalization Approach}
        \label{fig:architecture}
    \end{minipage}
\end{center}
\vspace{0.035 in}
\end{figure*}

When a large population of users is considered, there can be users who are different from each other as well as users with certain similarities. With the proposed technique, we aim to discover similar users for a target user and categorize them into a group (i.e., the community of the target user) in order to increase the number of data points in the training dataset when compared to training a user-level model. This is because gathering a large amount of data from a single user can be time-consuming, and it also allows higher accuracies as compared to population-level models \cite{kao2020user, jiang2018towards}. (The usage limitations of the user-level models because of the number of data points in the negative class and why this personalization technique is proposed for this specific inference task will be discussed in more detail in Section~\ref{subsubsec:ulm} and Section~\ref{subsubsec:inference_results_compare}). 
A high-level architectural view of the approach we used to infer mood-while-eating is shown in Figure~\ref{fig:architecture}. The approach consists of a user-level data aggregation method and user similarity matrix calculation as described in Section~\ref{sub:user_similarity_detection} and a community detection mechanism described as described in Section~\ref{sub:community_detection}. The purpose of the community-based personalization approach is to discover similar users for a given target user based on their behavioral and contextual data. 


\subsubsection{Obtaining the User Similarity Matrix}\label{sub:user_similarity_detection}


\paragraph{User-based Data Aggregation}\label{sub:user_based_data_aggregation}


First, to quantify the similarity between users, we use a mean-based data aggregation method similar to \cite{mitani2006local}. As given in Algorithm~\ref{alg:algorithm_user_based_data_aggregation}, for each user, we first filter out the data points of that user from the dataset ($D_{u}$) using the user id. Then we calculate the mean for each feature and generate a feature vector ($u_{aggr}$) for each user, by considering all the available data points. Hence, the feature vector of each user would have one value for all features in the dataset. Then, the feature vectors were included in the user-based aggregation matrix ($U_{aggr}$). This matrix provides an overview of all the users in the dataset and a summary of their features. In addition, this representation allows comparing users based on their feature vector.



\paragraph{User Similarity Matrix}\label{sub:user_similarity_matrix}



By using $U_{aggr}$ matrix, the next step is to calculate similarities between users. When we consider two vectors, the similarity between them can be calculated with the cosine similarity \cite{li2019improved}. Consider two aggregated user vectors $u1_{aggr}$ and $u2_{aggr}$ of randomly selected user1 and user2, respectively. Then we can find the similarity between those two users with Formula ~\ref{eqn:eqn_cosine} \cite{li2008mining}, where $i$ is the $i^{th}$ column index of the $u_{aggr}$ (i.e. $i^{th}$ feature of $F$).

\begin{equation}\label{eqn:eqn_cosine}
Sim_{cosine} = cos(\Theta) = \frac{A\cdot B}{\left \| A \right \|\left \| B \right \|} = \frac{\sum_{i=1}^{n} A_{i}\times B_{i}}{\sqrt{\sum_{i=1}^{n}(A_{i}^{2})}\times\sqrt{\sum_{i=1}^{n}(B_{i}^{2})}} = \frac{\sum_{i=1}^{|F|} u1_{aggr_{(i)}}\times u2_{aggr_{(i)}}}{\sqrt{\sum_{i=1}^{|F|}(u1_{aggr_{(i)}})^{2}}\times\sqrt{\sum_{i=1}^{|F|}(u2_{aggr_{(i)}})^{2}}}
\end{equation}




This similarity value between the two users suggests how close they are based on their smartphone sensing features and self-reports. We calculate this metric for all user pairs and represent it in a matrix of dimensions $|U|^{2}$. For each user pair, this value suggests how similar they are, where similarity increases when going from 0 to 1 (this is after normalizing the original -1 to +1 scale). Similar users to a target user can be selected using this metric. 


\subsubsection{Community Detection}\label{sub:community_detection}


In this section, we discuss the approach of threshold selection (Section~\ref{sub:threshold_selection}), where we select different community sizes based on a tunable threshold value and community detection (Section~\ref{sub:user_community_detection}). %Finally, we describe how the final dataset is created.



\paragraph{Threshold Selection}\label{sub:threshold_selection}

We use a threshold ($th$) to filter users similar to the target user. Depending on the value of the threshold, the size of the community would differ. For example, if $th = 0.85$, we take all the users who have similarity values equal to or greater than 0.85 with the target user as the community. Hence having the threshold at zero keeps all the other users in the community (similar to a population-level model), and we can increase the threshold to reduce the number of users in the community. While this makes the community much smaller, it also makes it much more similar to the target user. On the other hand, increasing the threshold helps to remove some users from the training set, who could have been noisy otherwise. Increasing the $th$ would affect the resulting dataset in two ways. First, it would reduce the number of users in the community, hence leading to comparatively smaller datasets for training models. Second, it is made sure that the selected data points are coming from similar users. Hence, depending on the chosen $th$, it could increase or decrease the size of the resulting dataset, hence affecting the accuracies of any model, trained on the dataset. In our experiment, we used a range of $th$ values to obtain accuracies for all users.


\paragraph{Community Detection}\label{sub:user_community_detection}


Depending on $th$, for each user, the number of similar users ($|U_{u_{t}}|$) might vary. As stated in the Algorithm~\ref{alg:algorithm_user_community_detection}, $Sim_{u_{t}}$ for each user is a vector with the dimensions of $1 \times (|U|-1)$, which contains the similarity matrix calculated for target user $u_{t}$, with other users in the dataset (i.e. $U \textbackslash \{u_{t}\}$). When iterating through similarity values for the target user, $Corr_{u}$ which is a similarity value of the target user with another user, is compared against $th$ to decide whether the other user is included in the community of the target user. After the community is detected, training and testing of personalized models can be done using the community dataset.


==> 05-Results.tex <==
\section{Results}\label{sec:results_of_rqs}


\subsection{{RQ1: Generic and Context-specific Model Performance}}\label{subsec:result_rq1}


First, Figure~\ref{fig:context_specific_models} shows that the generic mood inference model (best performing random forest classifier) trained with data from a wide range of everyday life occasions displayed contrasting performance across activities performed while the self-reports were provided. On the one hand, the results indicate that in both population-level and hybrid approaches, activities such as Resting, Walking, and Sports (which correspond to Mood-While-Resting/Walking/Engaging in Sports) showed higher performance than the overall accuracies (PLM: 43.6\%, HM 50.3\%) against a baseline of 33\%. On the other hand, the model performed the worst across Eating, Studying, and Working (which correspond to Mood-While-Eating/Studying/Working). Interestingly, people tend to use phones while resting and walking, while it is not the case while eating, studying, or working, which are exigent activities. Sport is an exception, where even though it is an exigent activity for which there were not many mood reports, the model still performed decently well. Along this line, prior work has shown that mental well-being during work is an interesting aspect that is worth further investigation \cite{9953824Morshed}. However, as we have discussed previously, such studies do not exist for mood-while-eating. 

Next, Figure~\ref{fig:context_specific_models} shows the effect of having mood reports during eating events for the overall performance on the testing set and also the performance of the model only for eating reports in the testing set (Mood-While-Eating). Results indicate that when no mood-while-eating reports are present in the training set, mood-while-eating performance is 45.6\% and overall performance is 55.2\%. However, when increasing the number of mood-while-eating reports in the training set, performance for mood-while-eating reports in the testing set increases to 47.8\%. This could be because more representation of mood-while-eating reports in the mood inference model training helped the model generalize better to mood-while-eating events in the testing set. Interestingly, when adding more mood-while-eating reports to the training set, the overall performance declined by around 3\% to 51.3\% before the curve got plateaued. This means that even though the number of data points for training the model increased, it did not work well for the overall performance because all the data points came from a similar context (i.e., mood-while-eating). This, in turn, would make the tree-based model learn representations for such contexts better than other contexts, leading to declining performance for other contexts at the expense of increasing performance for mood-while-eating events in the testing set. 

In summary, in response to \textbf{RQ1}, our findings indicate that generic models for mood inference do not exhibit consistent performance across various situated contexts. This could be attributed to the fact that self-report data may not be equally captured across all daily situations and that the ease of learning mood may vary depending on the context, such as during eating, studying, or working. Furthermore, our analysis revealed that an increase in the representation of mood-while-eating reports in the training set for the mood inference model led to improved performance on mood-while-eating reports in the testing set. However, overall performance declined, highlighting the challenge of generalizing to different situated contexts. These results suggest the need for context-specific models or better domain generalization techniques for mood inference in order to improve the accuracy of continuous mood tracking in mobile food diaries and health applications.

\begin{figure*}[t]
\begin{center}

    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/blank.png}
        \caption{}
        \label{fig:context_specific_models}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[t]{0.34\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/blank.png}
        \caption{}
        \label{fig:changing_eating_events}
    \end{subfigure}
    
    \caption{(a) This shows the context-specific accuracies of the generic mood inference model trained for MUL for approaches PLM and HM. (b) This shows the overall mood inference accuracy (All) and accuracy for eating events (Mood-While-Eating) when the number of mood-while-eating reports in the training set changes, with HMs for MUL.}
    \label{fig:context_specific_models}

\end{center}
\vspace{-0.2 in}
\end{figure*}



\subsection{{RQ2: Mood-While-Eating Inference}}\label{subsec:result_rq2}

\subsubsection{{Population-Level and Hybrid Model Results}}\label{subsubsec:inference_results_plm}


The results of the PLM and HM techniques are summarized in Table~\ref{tab:inference_results_pop_loo}. PLM accuracies were not sufficiently high. The highest accuracy obtained for the MEX dataset was 36.9\% using the RF, which is 3.6\% higher than the baseline accuracy. And for the MUL dataset, the highest was 43.6\% with the RF model type, which was 10.3\% higher than baseline accuracy. Model types such as NB, and SVC did not perform well with both datasets and the accuracies were lower than the baseline. The authors of \cite{pratap2019accuracy, kao2020user, xu2021leveraging} have mentioned the averaging effect in PLMs. Hence, In summary, the PLM approach did not perform well for the three-class inference task regardless of the data or model type. In addition, the HM results in both datasets show an increment in performance with the hybrid model type. The best accuracy from the HM approach is 64.0\%, which is an increment of nearly 27\% than PLM.
 
\begin{table}[t]
        \small
        \centering
        \caption{\textcolor{new}{Mean (\={A}) and Standard Deviation (A$_{\sigma}$) of inference accuracies, calculated using five models for the PLM and HM of mood inference task: \={A} (A$_{\sigma}$), F1.}}
        \resizebox{0.7\textwidth}{!}{%
        \begin{tabular}{l l l l l l l}

        \rowcolor{gray!10}
        \textbf{Feature Group}& 
        \textbf{} &
        \textbf{} &
        \textbf{PLM}&
        \textbf{}&
        \textbf{}&
        \textbf{HM} 
        \\

        %\arrayrulecolor{gray!15} 
        %\specialrule{6pt}{0pt}{-6pt} 
        
        \arrayrulecolor{black}
        \cmidrule{2-6}

        %\rowcolor{gray!15}
        \textbf{(\# of Features)}& 
        \textbf{RF} &
        \textbf{NB} &
        %\textbf{GB} &
        \textbf{SVC}&
        \textbf{XGB}&
        \textbf{AB} &
        \textbf{RF}
        \\
        
        %\rowcolor{gray!15}
        \textbf{}& 
        \textcolor{new}{\={A} (A$_{\sigma}$) }&
        \textcolor{new}{\={A} (A$_{\sigma}$)}&
        %\textcolor{new}{\={A} (A$_{\sigma}$), F1 }&
        \textcolor{new}{\={A} (A$_{\sigma}$)}&
        \textcolor{new}{\={A} (A$_{\sigma}$)}&
        \textcolor{new}{\={A} (A$_{\sigma}$)}&
        \textcolor{new}{\={A} (A$_{\sigma}$)}
        \\

        \hline 
        
        
        Baseline &
        33.3 (0.0) & % RF
        33.3 (0.0)& % NaiveBayes
        %33.3 (0.0), 33.3 & % GradienBoost
        33.3 (0.0) & % SVC
        33.3 (0.0) & % XGBoost
        33.3 (0.0) & % AdaBoost
        33.3 (0.0) %HM
        \\

        \arrayrulecolor{Gray}
\hline 
        
        MEX (40) & 
        36.9 (11.9)& % RF
        20.8 (8.2)& % NaiveBayes
        %32.1 (12.4), 35.4 & % GradienBoost
        20.4 (4.1) & % SVC
        30.4 (11.5)& % XGBoost
        31.2 (13.4) &% AdaBoost
        64.0 (20.8)  % HM
        \\
        
        % \cmidrule{1-7}

        \arrayrulecolor{Gray}
\hline 
        
        MUL (114) &
        43.6 (15.6) & % RF
        23.0 (10.6) & % NaiveBayes
         % & % GradienBoost
        32.5 (14.8) & % SVC
        41.0 (15.5) & % XGBoost
        37.9 (17.6) &% AdaBoost
        50.3 (20.6) % HM
        \\
        
    
        
        \hline 
        
        \end{tabular}}
        \label{tab:inference_results_pop_loo}

\end{table}






\subsubsection{User-Level Results}\label{subsubsec:ulm}

Even though we did not report results for user-level models (ULM), we conducted experiments with them for both datasets. ULMs are models that only use the target users' data in both training and testing with a 70:30 split (refer Table \ref{table:keywords_explaination} for explanation). However, the number of users for whom experiments could be carried out was fairly low because there was a low number of users with enough data to be split into training and testing sets. For example, in the MEX dataset, if we consider the number of classes represented in the dataset for each user, there are four users with data from only one class (only positive or only neutral), 32 users with data from only two classes (only two classes out of positive, negative, and neutral), and 25 users with data from all three classes (all positive, negative, and neutral). Hence, a generic ULM can only be built for these 25 users. However, as shown in Figure~\ref{fig:ulm_users}, the number of users with a high number of negative class labels decreases significantly when the number of labels is increased. For example, there are 16 users with at least two negative class labels, and it goes down to 4 users with at-least eight negative class labels. However, when data is split into training and testing, there might not be enough labels. Moreover, in the MUL dataset, the same issue can be identified, where there was a lesser percentage of negative class labels compared to the MEX dataset, which makes it more difficult to build user-level models using MUL dataset. Due to these reasons, ULMs can not be trained for a majority of users under reasonable assumptions. For the purpose of understanding, with an arbitrary negative label count of 6, we could train ULMs with the MEX dataset for six users with 70:30 training and testing splits and achieve an accuracy of 73.5\% with passive sensing modalities.

\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
    \centering
    \includegraphics[width=\linewidth]{images/ULM_users.png}
    \caption{MEX dataset: Distribution change in no. of users with the increase of no. of data points in the negative class.}
    \label{fig:ulm_users}
  \end{center}
\end{wrapfigure}

Overall, these results of \textbf{RQ2} suggest that, even though model types such as population-level, hybrid, and user-level can be used to infer mood-while-eating, either they lack performance or the model cannot be used with a large number of users due to lack of data.





\subsection{{RQ3: Mood-While-Eating Inference Using Community Based Personalization Approach}}\label{subsec:result_rq3}

\subsubsection{{Community-Based Model Results with Changing Thresholds}}\label{subsubsec:inference_results_ulcm} 

\begin{figure*}[t]
\begin{center}

    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/th-vs-acc-MEX.png}
        \caption{MEX dataset}
        \label{fig:clm_th_mex}
    \end{subfigure}
    %\hfill 
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/th-vs-acc-MUL.png}
        \caption{MUL dataset}
        \label{fig:clm_th_mul}
    \end{subfigure}
  
    \vspace{-0.1 in}
    \caption{Mean accuracy values(column values in the graphs) calculated using the random forest for CBM for multiple threshold values [No. of Users] and averaged community sizes (line values in the graphs)}
    \label{fig:clm_threshold_vs_acc}
\end{center}
\vspace{-0.2 in}
\end{figure*}

Figure~\ref{fig:clm_threshold_vs_acc} summarized the results of the CBM approach with MEX and MUL datasets.  Since RF models performed relatively well with the CBM approach compared to other classification model types and considering space limitations, we only discuss results obtained from RFs from here onwards. Both Figure~\ref{fig:clm_th_mex} and Figure~\ref{fig:clm_th_mul} show results of models when the threshold ($th$) value is increased from 0.85 to 0.99. Even though we obtained results for other threshold values ranging from 0 to 0.99, we only included threshold values that showed high variations in terms of accuracies, average community size, and the number of people to which the inference can be applied [No. of Users]. The point to note is that in these cases, the same threshold has been used on all users, which is not ideal. For example, for the MEX dataset, accuracy increases to a maximum of 79.4\% (at $th = 0.98$) and decreases afterward. This is mainly because as the threshold increases, the number of people in the community decreases, leading to a low number of samples for training models for a target user. This could decrease model performance. On the other hand, as $th$ increases, the similarity of users increases, hence leading to more similar data samples for a target user. This could increase model performance. Hence, the threshold value performs a trade-off between these two aspects. Even though there is no noticeable accuracy increase in MUL dataset with the increase in threshold values as the MEX dataset, similar behavior can be identified. In addition, we mention the number of users for which models can be trained using the approach for different thresholds. While a  $th=0.85$ allows creating models for 60 users in the MEX dataset,  $th=0.99$ only allows models for two users. The reason for this again is that for many users, there is no community at such high thresholds. 




In the rightmost column (MAX), we use different thresholds for different users, and the average threshold values for all the users, are given within brackets (ex: th=0.70). We empirically found the ideal threshold for each target user that yields the highest accuracy for the inference. Since the community size decreases when we increase the threshold, in order to build a model for a target user, there should be users with similarity values greater than the given threshold. MAX column summarizes the average results for such different thresholds. These are the best accuracies that we could expect when CBMs are deployed. For example, the accuracy value 80.7\% obtained for the MEX dataset (rightmost column) represents an average of maximum accuracies obtained for all the users. The 0.78 threshold value represents the average of threshold values associated with those accuracy values for each user. For the MUL dataset, the maximum accuracy obtained was 65.9\% with an average threshold of 0.70. Therefore, with CBMs, sensors performed reasonably well showing the potential of making mood inferences for eating occasions just using sensor data. Moreover, while such adaptive thresholds increased the overall accuracies, they also allowed the creation CBMs for all 61 users in the MEX dataset and 263 users in the MUL dataset.









\subsubsection{{Comparison of Approaches}}\label{subsubsec:inference_results_compare}


\begin{figure*}[t]
\begin{center}
    \begin{minipage}[t]{\textwidth}
        \centering
        \includegraphics[width=0.5\textwidth]{images/plm-hm-ulcm.png}
        \caption{Mean accuracies calculated using the random forest for the PLM and HM of mood detection task for all the users and Maximum mean accuracies for CBM calculated for all the users. }
        \label{fig:plm_hm_ulcm_comparison}
    \end{minipage}
\end{center}
\vspace{0.035 in}
\end{figure*}


The results of population-level, hybrid, and community-based approaches obtained with RFs for both MEX and MUL datasets are shown in Figure~\ref{fig:plm_hm_ulcm_comparison}. Compared to PLM, HM shows higher accuracies, supporting the idea that personalization gives better results than classic population-level leave-one-out methods. 

In real-world mHealth applications, it is difficult to capture large amounts of data from users \cite{kao2020user, jiang2018towards}. This is the main drawback of user-level models (i.e. the model is trained and tested by splitting the target user's data into two splits), even though they provide reasonably high accuracies. This MEX dataset was collected from the users for a reasonably long time period (close to 30 days). However, the number of collected data points was not sufficient to build a user-level model for many users because of the lack of negative class labels. The same goes with MUL dataset where the number of negative class labels in the dataset is not sufficient to build a 3-class model for most of the users. Additionally, there is a possibility of over-fitting user-level models to the target user when training the model using only the user's data because the model does not even account for intra-user variability, let alone inter-user variability. Hence, if the user's behavior changes with time, there is a chance of not being able to predict the mood correctly with the previously trained user-level models.

According to Figure~\ref{fig:plm_hm_ulcm_comparison}, the CBM shows better performance compared to the other two approaches for both datasets. Specifically, compared to HM, CBM accuracy was increased by over 15\%. In contrast to the user-level models we mentioned earlier, where each user needs to have a reasonable amount of data points in order to build a user-level model, this similarity-based approach can be used to build models for a high number of users, because the selected community of each user contains a comparatively higher amount of data which can be used to build the model. Furthermore, unlike user-level models, the machine learning model that had been built for each user shows robustness against behavioral fluctuations because the training split contains data from different users, which helps to avoid over-fitting. Hence, the CBM approach has the ability to capture both the inter-personal and intra-personal diversity of a target user. Moreover, with CBM approach the community of the selected user would be adjusted to the user's behavior change with the context around them.  
For the same set of users in MEX dataset, PLM and HM performed worse than CBM, again showing the benefit of selecting a similar community to train a model.



As shown in Figure~\ref{fig:clm_threshold_vs_acc}, we can observe that the average community sizes decrease with the increase of threshold value. And it can be observed that each user has different threshold values and community sizes. To get an overall idea of the community size variability with multiple threshold values, a heat map generated using the MEX dataset is given in Figure~\ref{fig:fi_heat}. It shows how the community size is reduced when the threshold is increased. Figure~\ref{fig:fi_acc} shows the average of accuracies obtained for all the users. It clearly depicts that the accuracy slightly increases with the threshold. This concludes that for any user, when the threshold is increased, the community size of that user decreases and the accuracy might increase. However, after high thresholds, the accuracy drops off again because of lack of members in user communities. A cumulative density function (CDF) figure for maximum accuracies is included in Figure~\ref{fig:fi_pdf_cdf}. Please note that considering the space limitation we have only included the distributions of MEX dataset.


\begin{figure*}[t]
\begin{center}

    \begin{subfigure}[t]{0.38\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/heatmap.png}
        \caption{Community size of users with threshold.}
        \label{fig:fi_heat}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[t]{0.30\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/mean_accuracy_w_th_G4.png}
        \caption{Random Forest Accuracy with threshold.}
        \label{fig:fi_acc}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/cdf.png}
        \caption{CDF of Accuracy}
        \label{fig:fi_pdf_cdf}
    \end{subfigure}
    \hfill 
    
    \caption{Distributions of CBM using MEX dataset: (a) How the community size of each user changes with threshold $th$; (b) How the mean accuracy of the Random Forest model changes with threshold $th$; (c) Cumulative Distribution Function (CDF) of Accuracy.}
    \label{fig:feature_importance_pers2}
\end{center}
\vspace{-0.2 in}
\end{figure*}






\subsubsection{{Feature Importance for Mood Detection}}

\begin{figure*}[t]
\begin{center}
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{images/fi_clm_mex.png}
        \caption{Gini Feature Importance values of top 20 features generated using Random Forest for CBM of MEX dataset}
        \label{fig:fi_clm_mex}
    \end{minipage}
    \hfill 
    \begin{minipage}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\linewidth]{images/fi_clm_mul_all.png}
        \caption{Gini Feature Importance values  of top 20 features generated using Random Forest for CBM of MUL dataset}
        \label{fig:fi_clm_mul}
    \end{minipage}
\end{center}
\vspace{-0.2 in}
\end{figure*}


In this section, we explore the gini feature importance for mood inference generated using Random Forest classifiers for CBM with passive sensing features using MEX and MUL datasets. In Figure~\ref{fig:fi_clm_mex} and Figure~\ref{fig:fi_clm_mul}, we plot those values of top features in MEX dataset and MUL dataset respectively. We can identify that some features like the radius of gyration, battery level and time of the day have higher values compared to the rest in CBM in MEX dataset, where features that represent time of the day such as minutes elapsed, day, hours elapsed have higher values in MUL dataset. On one hand, higher feature importance value in radius of gyration suggests that distances traveled closer to eating episodes had an association with the mood of the user or vice versa. For example, some studies have shown that user might travel long distances during the day regardless of the geographical location, in order to find food \cite{ma2015food, kerr2012predictors}. Further, there is a considerable correlation between mobility patterns, time of the day, and the semantic location with psychological constructs such as depression \cite{canzian2015trajectories}. This may explain this finding. Battery level is another feature that has shown high feature importance across all model types in MEX dataset. Even though there is no clear explanation as to why this could happen, prior work too have suggested that battery level and charging events could be informative regarding eating and drinking events \cite{Bae2017, Meegahapola2021OneMoreBite}. This could be because battery level provides contextual information regarding the location the person is in \cite{Bae2017, Meegahapola2021Survey}. In fact, time of the day has shown to be useful in eating behavior-related tasks \cite{Biel2018, Meegahapola2021OneMoreBite}. In addition, hour of the day is a reasonable feature to estimate mood, where negative moods increase when going from morning to evening \cite{mislove2010pulse}. Feature importance values corresponding to the accelerometer showed significantly higher values in MEX dataset, suggesting that physical activity levels around eating episodes could be informative about moods, whereas some studies have presented that mood can cause the daily activity levels \cite{roshanaei2009longitudinal}, and these activity levels can be detected using acceleration data \cite{rabbi2011passive}. Moreover, it is also observed that screen events in MUL have moderate feature importance values. Sano et al. \cite{sano2013stress} also used mobile phones to show that screen events have correlations with the stress levels of users. These results support the idea that mobile phone sensor data could play a role when it comes to inferences of mood-while-eating with only passive sensing data.


In summary, these results of \textbf{RQ3} suggests that personalization is a key component in achieving better performance in mood-while-eating inference task. The proposed community-based technique helps to overcome the challenges such as the lack of individual data and the cold-start problem. 


==> review-old/00-responses.tex <==
\textcolor{black}{\begin{center}\textbf{Reviews and Responses}\end{center}} 


We thank the reviewers for their valuable comments that were helpful in reshaping the paper. In this document, we have listed all the review comments and our responses, including the changes that were made. To facilitate reading, we use \textcolor{red}{\textbf{red}} color to indicate the original comments, \textcolor{black}{\textbf{black}} color to provide our responses, and \textcolor{gray}{\textbf{gray}} color to indicate the concrete changes made to the paper. Under concrete changes, we used \textit{[…]} mark to indicate shortened sections. The complete text of such sections can be found in the manuscript. Major changes done in the manuscript are marked with \textcolor{blue}{\textbf{blue}} color. \\

% \textcolor{blue}{Note: Will add the figures with enlarged text to the paper.}

% ==================REVIEW -REPLY=================

% \textcolor{green}{started or ongoing}

% \textcolor{blue}{done}

% ==================PAPER========================

% \textcolor{yellow}{remove}

% % \textcolor{new}{new additions in the paper} 
% \textcolor{red}{new additions and changes}

% \textcolor{orange}{need changes}


\input{review/R0-summary}
\input{review/R1}
\input{review/R2}
\input{review/R3}

\newpage



==> review-old/R0-summary.tex <==
\textcolor{red}{\begin{center}\textbf{Summary meta-review}\end{center}}


\textcolor{red}{The reviewers find the motivation and the scope of the paper interesting and appropriate. However, several concerns raised on the study need to be addressed before accepting the paper. Hence, a major revision is being recommended.
In the major revision version of the paper, please address all the concerns raised by the reviewers. Some key ones are listed below:}\\

\textcolor{red}{1.      Clarify if SMOTE was not applied to the test set and justify that there is no information leakage. (R2) If SMOTE is used in the test set, it is recommended that authors redo the evaluation without applying SMOTE in the test set to avoid any bias.}\\

We have now clarified the point about SMOTE in the revised version. Please refer to the response to Comment R2-10 on page 9 of the response.\\


\textcolor{red}{2.      Add some discussion (and justification) on the motivation of the study, usability, and practical use of the approach. Particularly who are the target users, in which context the approach is usable, how to use it, etc.  (R2,R3).}\\

We have now added more motivation and changed sections, in the introduction and related work sections. Please refer to the response to Comment R2-19 on page 14 of the response.\\

\textcolor{red}{3.      The paper needs restructuring and clarifying its novelty, motivation, dataset, and result discussion. (R2,R3)}\\

We restructured the paper to improve readability. Please refer to the response to Comment R2-2 on page 6, Comment R2-3 on page 7, and Comment R3-1 on page 16 of the response.\\

\textcolor{red}{4.      Justify and discuss in detail the design choices of the study and evaluations performed. See comments from R3.}\\

We added more details to the relevant sections. Please refer to the response to Comment R3-5 on page 17 of the response.\\

\textcolor{red}{5.      The hybrid method is identified as the most effective one. However, several reviewers’ showed concerns about this generalizability (R1,R2). Justify in detail about the generalizability of the Hybrid method.}\\

We added more details regarding the hybrid method and provided details regarding the generalizability concerns. Please refer to the response to Comment R1-2 on page 4 of the response.\\

\textcolor{red}{6.      Justify with prior study references or insights if mood can be differently impacted/experienced while eating vs. on-other-contexts. Justify the problem (R4). Emphasize the importance of studying mood while eating in the introduction and abstract (R2).}\\

We added more details regarding this to the introduction, related work, and abstract. Please refer to the responses to Comments R2-2 and R3-2 on pages 6 and 16 respectively, of the response.\\

\textcolor{red}{7.      Dataset: Justify the reason why Mexico is specified in the evaluations. Include a detailed discussion about the datasets used (including demographic information). (R2) Explain clearly in the data collection section how eating events were determined.}\\

We included more details about the datasets, and clarified the reasons for having two separate datasets. Please refer to the responses to Comments R2-1, R2-9, and R2-14 on pages 6, 9, and 12 respectively, of the response. \\

\textcolor{red}{8.      Explain the terms used in the text.}\\

We addressed this comment by introducing and referring to the terms, earlier in the paper. Please refer to the responses to Comments R1-3 and R2-13 on pages 4 and 12 respectively, on the response. \\

\textcolor{red}{9.      Justify why, even having two different test sets, a comparison between population-level, personalized, and community models is valid.}\\

We added more justification, referring to past work regarding the validity of the techniques. Please refer to the response to Comment R2-4 on page 7 of the response. \\

\textcolor{red}{10.     Alongside accuracy, other additional metrics that are justified when data is imbalanced need to be used. Include F1-score, precision, and recall in the analysis. The data imbalance issue is making the results not properly interpretable.}\\

We added the F1 score to all the main results. Please refer to the response to Comment R1-3 on page 4 of the response. \\

\textcolor{red}{11.     Include the mean and standard deviation, median and IQR, of eating reports per participant in the evaluation.}\\

We added these details. Please refer to the response to Comment R2-7 on page 9 of the response. \\

\textcolor{red}{12.     explain why using 90\% of the population and 30\% of a user’s data enhances robustness. Give reference if it is an established approach from literature.}\\

We clarified details regarding sub-sampling and the rationale. Please refer to the response to Comment R2-11 on page 10 of the response. \\

\textcolor{red}{13.     Address the issues about the tables, figures, and typos pointed out by the reviewers.}\\

We addressed all of these concerns. Please refer to the responses to Comments R2-6, R2-8, R2-16, and R2-18, on pages 8, 9, 13, and 14, respectively, on the response. \\


==> review-old/R1.tex <==
\newpage 
\textcolor{red}{\begin{center}\textbf{Reviewer 1 }\end{center}}

\textbf{Recommendation: Minor Revision}\\

\textcolor{red}{\textbf{Comments:}}\\
\textcolor{red}{The paper presents a comprehensive analysis of the relationship between mood and eating with mobile sensing data. The authors conducted experiments with the Mexico dataset and with the multi-country dataset using passive sensing data. The paper is well written, and the research questions are clearly stated and explained.}\\

\textcolor{red}{\textbf{Possible improvements:}}\\


\textcolor{red}{\textbf{Comment R1-1 : } }
\textcolor{red}{The technical contribution of the paper is limited, as the claimed contribution of a novel community-based approach for personalization by building models have been widely explored in the literature.}\\

Sorry if the technical contribution of the paper was not clear. To the best of our knowledge, there are two key contributions of this paper. 
\\

First, model generalization is an important area of research. In our prior work, we have delved deeply into this phenomenon, with a specific focus on mobile health sensing \cite{meegahapola2023generalization, KarimAssi2023, nanchen2023keep, kammoun2023understanding}. There are two primary notions of generalization \cite{jones2020selective, meegahapola2023generalization}: i) generalization of models to a different target domain; ii) sub-sample/context generalization, which involves generalizing a model to a sub-sample or a population within the source domain. We explored the first notion of generalization in the context of mobile health sensing \cite{meegahapola2023generalization, KarimAssi2023, nanchen2023keep, kammoun2023understanding}, as did other recent studies \cite{xu2023globem}. However, the second notion of generalization, even though extensively studied in general machine learning literature \cite{jones2020selective, yang2023change}, has not been thoroughly investigated in the field of mobile health sensing. We believe that understanding this aspect of generalization is crucial for the development of future mobile health sensing systems that can operate effectively across diverse contexts. This is the focus of our investigation in Research Question 1. In response to this comment, we have rephrased and emphasized the novelty of our work in Section 1 and Section 2.
\\

Second, while there have been previous studies examining similarity-based personalization approaches, we believe our work brings a novel contribution. To clarify, there are no prior studies that have employed the same community-based approach to address the challenge of having a limited number of data points in the training set. Kao et al.\cite{kao2020user} conducted a study that uses a user-based collaborative filtering method where health predictions are made without relying on historical data from the selected user. In this study, the user is assigned to a cohort, and the health predictions are made by selecting a user with similar characteristics. This study differs from our study in two aspects: 1. we select a group of users who are similar to the selected user. 2. the number of users in the selected group can be changed using the defined threshold value. Another study used community similarity networks, where all the users are considered in training models based on the weighted similarity \cite{lane2011enabling}. With our method, we identify a community of users with similar behavioral and contextual patterns for each individual, effectively providing a larger training dataset. Similarities between users are calculated using cosine similarity, and we have the flexibility to adjust the size of the community by choosing appropriate threshold values. The model's performance is dependent on the selected user's community size.\\

In the revised version, we have highlighted these novelties, in the introduction (section 1) and related work (section 2).

% \cite{kao2020user} - user-based collaborative filtering, 
% health predictions without historical data from the user - used other users' data, 
% cohort similarity using health labels , clustering algorithm, select a user who is similar

% lane2011enabling - add inter-person similarity measurements to the classifier training
% every user have unique classifier tuned to their own characteristics 
%  all the users are considered and calculated the weighted similarity values
% population diversity problem address


% \cite{xu2021leveraging} - user-item matrix
% collaborative filtering - used in recommendation systems
%  person correlation
%  feature selection for users on 
% related group - target user - 
% relevance score to find the group of users with time
% majority voting
% 

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 2.5, p.08 -> "In summary, our technique is model-agnostic and does not assign a user to a pre-defined community. Instead, it finds a unique community for each target user, the size of which can be adjusted using a tunable threshold parameter. This accounts for both inter-personal and intra-personal variability that could affect model performance. Furthermore, our technique effectively addresses the challenge of low data points in the training set by identifying similar users and building a community for the selected user."}}}\\

{\small\textit{\textcolor{gray}{Section 1, p.02 -> "Recent studies within the domains of mental well-being and mobile sensing have highlighted the lack of generalization of models in various contexts, including different countries and time periods, due to distributional disparities in data, commonly referred to as distribution shift...Hence, more specifically, prior work has rarely examined the generalization performance of sensing-based mood inference models during specific contexts in which data were collected, such as eating, studying, working, etc., that are sub-samples of data pertaining to different contexts."}}}\\




\textcolor{red}{\textbf{Comment R1-2 : } }
\textcolor{red}{ The authors stated that the hybrid modeling approach may be a more effective method for mood-while-eating inference. They mentioned that the hybrid models (HM) resulted in an accuracy improvement of 27.4\% for the Mexico dataset. Although this result is intriguing, however I am not certain about the generalizibilty of such hybrid models. For example, how would the model behave if it is trained on one set of population and tested on a different unseen group of population. }\\

% In addition, hybrid method cannot be for generalizability. Hybrid model is trainined using a 

% Generalizability for diff datasets is a diff area - 

% Mention past studies
% \cite{meegahapola2023generalization}
% \cite{xu2023globem}
% \cite{KarimAssi2023}

% Distribution shift
% Sub population generalizability - our paper - for diff contexts
% Add to discussion
% Sub population shift
% https://youtu.be/5tidNjeVG8s?si=8ODRCQjxpoxNTF8b

% hybrid model is not for generalizability, but personalization for a given user

% Where we describe this model, say this in simple words explicitly.

% Distribution 2 sides (distribution shift): same dataset sub population & different population. Our aim is to just touch the sub population generalizability of this model

% Refer prior papers that mention generalizability for different populations. 
% https://dl.acm.org/doi/10.1145/3544548.3581190


The sentence provided under the Discussion section for RQ2, "These results suggest that the hybrid modeling approach may be a more effective method for mood-while-eating inference," may have been misleading. We appreciate the reviewer for pointing this out. The intended message for RQ2 was to compare the performance of the hybrid model to that of the population-level model and highlight that the hybrid model exhibits better performance in inferring mood while eating. Furthermore, there was a 7.4\% improvement in accuracy for the MEX dataset.\\

It is important to note that hybrid models cannot be generalized. Since these models are trained using a portion of the selected user's data, they are personalized for that specific user. As a result, hybrid models cannot be applied to other users or different populations.\\

Additionally, out-of-distribution generalizability to different datasets has been explored in previous studies \cite{meegahapola2023generalization, xu2023globem, KarimAssi2023}. However, this falls within a separate research area that is not the focus of our current study. Our paper specifically concentrates on sub-context generalizability, which involves assessing the ability of the models to generalize within the same dataset, to a particular group of samples. We have rephrased the discussion section's RQ2 to prevent any confusion.\\ 


\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 7.1, p.21 -> RQ2: "The performance of mood-while-eating inference models was assessed using both population-level and hybrid modeling approaches...Additionally, we discussed the challenges in training fully personalized user-level models across both datasets, primarily due to insufficient data in certain classes"}}}\\


\textcolor{red}{\textbf{Comment R1-3 : } }
\textcolor{red}{It would be great if the authors provided an F1-score analysis of all experiments, instead of showing only the accuracy improvements. For example, the authors mentioned that the development of the user-level models were hindered for many users because of the lack of negative class labels. The precision and recall performance of the models are not understandable based on the accuracy results.}\\

% [will add F1 results to results]
% [ we have random forest results with F1 score, can add this to paper]
% Table and final comparison results 

Thank you for this comment. In response to this review, we added the F1 scores to most of the main results sections. The results hold a similar pattern to that of the accuracy, in most cases. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Table 2 -> "Added the F1 scores" }}}\\

{\small\textit{\textcolor{gray}{Fig. 6 -> "Added a figure with F1 scores" }}}\\

{\small\textit{\textcolor{gray}{Section 6.2.2 p.18 -> "The results of population-level, hybrid, and community-based approaches obtained with RFs for both MEX and MUL datasets are shown in Figure 6a. The F1 scores of the three model types for both datasets are shown in Figure 6b. Compared to PLM, HM shows higher accuracies, supporting the idea that personalization gives better results than classic population-level leave-one-out methods" }}}\\

{\small\textit{\textcolor{gray}{Section 5.2.1 p.14-> "The results of the PLM and HM techniques are summarized in Table 2. PLM accuracies and F1 scores were not sufficiently high. The highest accuracy and F1 score obtained for the MEX dataset was 36.9\% and 36.7\% using the RF, which are 3.6\% and 3.4\% higher than the baseline performances respectively." }}}\\



==> review-old/R2.tex <==
\newpage 

\textcolor{red}{\begin{center}\textbf{Reviewer 2 }\end{center}}

\textbf{Recommendation: Major Revision}\\

\textcolor{red}{\textbf{Comments:}}\\
\textcolor{red}{This paper investigates the use of passive sensor data to infer mood while eating. It specifically looks at the generalizability of these models in larger populations, using a dataset from Mexico and eight other countries, and experiments with different approaches to personalization to improve generalizability. The paper finds that population-level and hybrid models fail, but community-based approaches to personalization improve model performance.
I found the motivation for this work to be justified in the paper, and the ideas around context and personalization interesting. These ideas could be a good contribution to this field, but I have some significant concerns around the execution and experimental design in this paper, specifically the machine learning methods and results presentation (see comments on SMOTE, data leakage, and variability across test sets). See point by point suggestions below. I hope the authors find these suggestions helpful for improving their work.}\\


%===============================================
%===============================================
%===============================================
\textcolor{red}{\textbf{Abstract}}\\

\textcolor{red}{\textbf{Comment R2-1 : } }
\textcolor{red}{Is there a reason why Mexico is specified, while the eight other countries’ data is grouped together? Would it be clearer and more consistent to say nine countries, with the N listed as the number of mood self-reports during eating? If this separation is explained later please also clarify in the abstract.}\\

% [ Can explain in dataset section] - and abstract
% 2 separate studies
% Change abstract

Sorry if the dataset description was confusing. The MEX dataset (from one country) and the MUL dataset (from eight countries) used in this study were collected from two different pilot studies. The MEX dataset was collected in 2019 \cite{Meegahapola2021OneMoreBite}, while the MUL dataset was collected in 2020 \cite{meegahapola2023generalization}. Both datasets contain sensor data and self-reported data. However, the data collection protocols and the captured features in the MUL and MEX datasets were different, making it impossible to combine the two datasets. Therefore, in our study, we treat the eight countries in the MUL dataset as one dataset and use the MEX dataset as another dataset. In response to this review, we have made some changes to describe the datasets in Section 3 and have also modified the Abstract accordingly.\\


\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Abstract p.01 -> "In this study, we sought to examine everyday eating behavior and mood using two separate datasets of college students collected from: i) Mexico (N = 84, 1843 mood-while-eating reports) in 2019 ii) eight countries (N = 678, 329K mood reports incl. 24K mood-while-eating reports) in 2020, containing both passive smartphone sensing and self-report data"}}}\\


\wageesha{{\small\textit{\textcolor{gray}{Section 3 p.09 -> "Not a lot of datasets exist to study the intersection of mood and eating behavior with mobile sensing data. Hence, we used two novel datasets collected from two separate studies. Further details about these datasets can be found in our previous works \cite{Meegahapola2021OneMoreBite} and \cite{meegahapola2023generalization}, respectively"}}}}\\


%===============================================
%===============================================
%===============================================
\textcolor{red}{\textbf{Introduction:}}\\

\textcolor{red}{\textbf{Comment R2-2 : } }
\textcolor{red}{The authors state “Despite the examination of context-agnostic mood inferences in prior studies, the effectiveness of such inferences in specific contexts, such as eating occasions, has not been explored before.”. I would incorporate the justification on why it is important to study mood while eating stated in the next few paragraphs (“great value to track holistic eating behavior” and “aid in the development of effective personalized interventions”) sooner in the work, and include this importance in the abstract. The context of mood while eating is initially stated without motivation, and until this point, I did not understand why mood while eating is an important context to study.}\\


% [Modify abstract and intro ]
Thank you for the suggestion. As the reviewer correctly said, there are many benefits of this inference, and in the previous version of the paper, we may have introduced them a bit later. However, in response to this review, we have revised the introduction and abstract sections to emphasize the importance of mood-while-eating earlier in the paper.\\


\textit{\textcolor{gray}{Concrete Changes :}}\\

\wageesha{{\small\textit{\textcolor{gray}{Abstract p.01 -> "Examining mood for a specific context, such as eating, will provide valuable insight for comprehensively understanding the eating behaviors of humans." }}}}\\

{\small\textit{\textcolor{gray}{Introduction p.02 -> "Mental well-being and eating behavior have been the subjects of numerous studies,.. " }}}\\



\textcolor{red}{\textbf{Comment R2-3 : } }
\textcolor{red}{Could the authors define in RQ3 what the “community-based model” is before stating this terminology? I realize it is in Table 1, but this table has not yet been referred to.}\\

Thank you for this comment. We modified the RQ3 accordingly. In addition, before RQs, we directed the readers to Table 1, to clarify that we use terminology from the tables in RQs and contributions. The community-based model, along with the other models and the main task, are properly defined in Table 1.
 \\
% [Modify RQ3 and Refer table when describing CBM ]

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Introduction p.03 -> "RQ3: What measures should be taken to tackle issues such as lack of individual data and cold-start problem in mood-while-eating inference, in building personalized models? Can a community-based model overcome such issues?" }}}\\

{\small\textit{\textcolor{gray}{Introduction p.03 -> "In light of these considerations, in line with the terminology provided in Table 1, we pose the following research questions." }}}\\



\textcolor{red}{\textbf{Comment R2-4 : } }
\textcolor{red}{In Contributions 2 and 3, is it appropriate to make statements comparing the population-level, partially personalized, and community models, given these approaches were tested using different test sets? How do we know that the model improvements are not simply because we’ve reduced the testing set size and made the problem easier? It would be clearer to state the accuracy of each model, without the comparators. Or, the authors show clearly align the test sets across each model.}\\

% [ justify why we selected random test data using past work]
% Same test cannot be tested
% Random test set  - past papers
% 1. cannot get the same test set for those models
% 2. Past papers also have done similar

%\lakmal{\textbf{[DONE WAGEESHA: I do not think the response to this comment clearly answers the reviewer. We have agreed with the limitation the reviewer pointed out and tried to justify the way we presented results by citing our own work--which does not make sense. However, what if the reviewer again thinks what we have done in past work is incorrect? So, it's good that you have also cited LiKamwa's work. Find some more similar work from others, and include them as references. In addition, try to think of a better justification. Some suggestions --> Maybe acknowledge that this is a limitation; find at least a few past studies from other authors (top-tier papers from good labs + professors) that this is the way it is. Add a few sentences in some places to acknowledge the differences in testing sets; highlight this as a LIMITATION in the discussion section. Reduce the number of places where we do comparisons of results, directly.]}}\\

We agree with the reviewer's comment regarding the importance of using the same test dataset to compare each model's performance. However, for our three approaches (PLM, HM, and CBM), it is not feasible to use the same dataset for testing. In the Population-Level Model (PLM), we employed a leave-one-out strategy, where the test set contains only the data of one user, and the training set comprises data from other users, excluding the selected user. In the Hybrid Model (HM), we adopted a partially personalized approach, where the test dataset includes a portion of the selected user's data and is tested against the remaining portion of the data. In the Community-Based Model (CBM), a segment of the user's data is added to the training set, along with data from the user's community. Furthermore, we had to select a random set of user data for personalizing the HM and CBM models, as we needed to run multiple iterations of the models and calculate the average accuracy. Therefore, in these three model types, the training and testing datasets cannot be the same. However, we still believe that with multiple iterations of running the experiments with multiple random samples, we aimed to provide a reasonable estimate of performance that would make the comparisons reasonable.\\



% \cite{likamwa2013moodscope} - model comparison - hybrid model,  all-user model
% \cite{hong2015toward} - model comparison - individual model, population model (LOO), multi-personlization and single-personlizatin comparison  
% \cite{chu2009personalized} - compare  aggregate level (population level), segmentation level (cluster of users) and individual level models



Additionally, similar approaches have been used in past work, where results from different model types were compared with each other. Likamwa et al. \cite{likamwa2013moodscope} compared the all-user model (testing with the user's data after leaving it out), the hybrid model, and the user-specific model in predicting mood and demonstrated that personalized models outperformed all-user level models. Moreover, Hong et al. \cite{hong2015toward} conducted a study on activity recognition, comparing the performance of individual-level, population-level, multi-personalization, and single-personalization models. Furthermore, Chu et al. \cite{chu2009personalized} carried out a study on personalized recommendation systems, employing aggregated level models (population level), segmentation level models (using clusters of users), and individual level models to compare the results among the various model types.\\


% In addition, the same approach was used in past work, where results from different model type were compared with each other to show that the personalized approaches perform well in given context. In one past work, the authors used population level models, hybrid model and user-level models where they used random test sets and compared the results across three model types  \cite{Bangamuarachchi2022Sensing}. Moreover, in another past work, the authors used  all-user model, hybrid model and user models in order to show the accuracy of the models increase when the number of data in the training set increase with the number of user data in the training set \cite{likamwa2013moodscope}. In these both studies the authors compared the results across multiple models types even thought the testing datasets contained different data. \\


Due to these considerations, in response to the reviewer’s comment, we have revised the "limitations and future work" section to include this specific limitation regarding the comparison of results and the need for caution in doing so.\\


\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 7.3 p.23 -> "Finally, another limitation of our study is the use of random test datasets to evaluate the performance of the Population-Level Model (PLM), Hybrid Model (HM), and Community-Based Model (CBM). Ideally, for a fair comparison of the results across each model type, it would be best to use the same test dataset. Nonetheless, due to the inherent differences in the model types, it is challenging to assess their performance using a uniform test dataset. For example, while the PLM is developed using a leave-one-out strategy, the HM and CBM incorporate personalization strategies." }}}\\




\textcolor{red}{\textbf{Comment R2-5 : } }
\textcolor{red}{Similar to my question in the abstract, why was the Mexico dataset tested separately from the multi-country dataset? If it is because the datasets could not be combined? Can this be stated upfront?}\\


Please refer to the response to Comment R2-1.\\

% [Edit data set section]

% \textit{\textcolor{gray}{Concrete Changes :}}\\
% {\small\textit{\textcolor{gray}{Introduction p.03 -> "" }}}\\



\textcolor{red}{\textbf{Comment R2-6 : } }
\textcolor{red}{Since accuracy is used to describe model performance, it would be helpful to list the percentage of positive, neutral, and negative samples in the abstract and introduction, so we have an understanding of the dataset balance and how that influences model accuracy.}\\

% edit abstract
% Imbalance dataset 
% `with the challenging unbalanced dataset`

Thank you for this suggestion. We modified the abstract and dataset sections in order to add more details about the dataset. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Abstract p.01 -> "Driven by how examining mood in specific contexts such as eating, can provide valuable insights into comprehensively understanding human eating behaviors, in this study, we analyzed everyday eating behavior and mood using two separate datasets of college students collected from: \textit{i)} Mexico (N$_{MEX}$ = 84, 1843 mood-while-eating reports with a label distribution of positive:51.7\%, neutral:38.6\% and negative:9.8\%) in 2019 and \textit{ii)} eight countries (N$_{MUL}$ = 678, 329K mood reports, including 24K mood-while-eating reports with a label distribution of positive:83\%, neutral:14.9\%, and negative:2.2\%) in 2020, which contain both passive smartphone sensing and self-report data.." }}}\\

{\small\textit{\textcolor{gray}{Fig. 1 -> Added the percentages of positive, negative, and neutral samples to the figure.}}} \\



%===============================================
%===============================================
%===============================================

\textcolor{red}{\textbf{Dataset Description}}\\

\textcolor{red}{\textbf{Comment R2-7 : } }
\textcolor{red}{Could the authors include the mean and standard deviation, or median and IQR, of eating reports per participant?}\\

% [ add the data to dataset section]

Mean was already present. We added the standard deviation of eating reports to the dataset section.\\

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 3.1 p.09 -> "with an average of around 30 eating reports per participant (standard deviation = 29.39)" }}}\\

{\small\textit{\textcolor{gray}{Section 3.2 p.10 -> "where 24k self-reports were associated with eating events, with an average of 92 per user (standard deviation = 58.88" }}}\\





\textcolor{red}{\textbf{Comment R2-8 : } }
\textcolor{red}{Figure 1 is a bit difficult to read, with small axes titles and ticks. Could these be enlarged? Also, in addition to the number of samples in each class (eg, positive), could the percentage of samples also be listed so the imbalance is obvious?}\\

% [ edit figure]

We added an edited version with enlarged text. We also included the percentage. The Y-axis shows the actual number of reports.\\

\textit{\textcolor{gray}{Concrete Changes :}}
\\

{\small\textit{\textcolor{gray}{Fig. 1 -> Edited the figure to make it more readable, by also including the requested percentages.}}}
\\




\textcolor{red}{\textbf{Comment R2-9 : } }
\textcolor{red}{In 3.2, “Data collection”, could the authors explicitly state how eating events were determined in the multi-country dataset? I think this is hinted at in the “Passive Smartphone Sensing and Self-Reports” section, but should be stated sooner.}\\


% [ add description to dataset section ]

Thank you for the suggestion. Eating Events were determined based on in-situ self-reports provided by phone app users. In those self-reports, they reported the food types that they ate, and contextual circumstances during the event occasion (e.g., location, social context, etc.) together with mood. As a response to this review, we added a more extensive description of the MUL dataset in the dataset section.\\


\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 3 p.10 -> "The passive sensing data were collected throughout the day [...] This helps to identify the eating moments of the user, the context around the user, and the aggregated passive sensing data of the eating moment" }}}\\




%===============================================
%===============================================
%===============================================

\textcolor{red}{\textbf{Methods}}\\

\textcolor{red}{\textbf{Comment R2-10 : } }
\textcolor{red}{The use of SMOTE for both training and down-sampled test sets is a bit concerning to me. Typically, SMOTE is used to balance training sets, but it is still necessary for the test set to match the distribution of data in the real world, otherwise generalizability is not really being tested (unless the authors have reason to believe the balanced distribution is the true distribution in the real world). In addition, I believe performing SMOTE on testing data would result in data leakage. Could the authors confirm if they applied SMOTE to the test set? If so, I do not think the results are valid, unless the authors rerun their experiments without applying SMOTE to the test set. Also, what is the “down sampling” being applied to the test set? See how SMOTE has been applied in prior work:}


\textcolor{red}{1. Aniruddh Raghu, Divya Shanmugam, Eugene Pomerantsev, John Guttag, and Collin M. Stultz. 2022. Data Augmentation for Electrocardiograms. Proceedings of the Conference on Health, Inference, and Learning, PMLR, 282–310.}

\textcolor{red}{2. Ruben van den Goorbergh, Maarten van Smeden, Dirk Timmerman, and Ben Van Calster. 2022. The harm of class imbalance corrections for risk prediction models: illustra tion and simulation using logistic regression. Journal of the American Medical Informatics Association: ocac093.}

\textcolor{red}{3. Daniel A. Adler, Fei Wang, David C. Mohr, and Tanzeem Choudhury. 2022. Machine learning for passive mental health symptom prediction: Generalization across different longitudinal mobile sensing studies. PLOS ONE 17, 4: e0266516.}\\

% \cite{raghu22adataaug}
% \cite{vanden2022}
% \cite{adler2022ml}

We thank the reviewer for suggesting these papers. We apologize if the sampling of the training and testing sets were not clear in the method section. We used SMOTE to up-sample the training set, and we down-sampled the testing set in order to balance the three classes (positive, negative, and neutral). We did not use SMOTE on the testing set as it is not a recommended approach. As a response to this review, we clarified our methodology. \\


\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 4 p.11 -> "Moreover, we employed the Synthetic Minority Over-sampling Technique (SMOTE) \cite{chawla2002smote} on training sets to up-sample and balance the dataset. SMOTE is used to generate new synthetic data points for the minority class using k-nearest neighbors \cite{raghu22adataaug, adler2022ml}. For testing sets, we down-sampled majority classes to achieve balanced datasets, establishing a baseline accuracy of 33.3\% in the three-class inference, for all experiments." }}}\\

{\small\textit{\textcolor{gray}{Section 7.3 p.23 -> " In this study, we employed SMOTE to up-sample and balance the training dataset. However, past studies have suggested that using SMOTE might not always enhance the accuracy of prediction models [137]. Therefore, future research should investigate the performance of models built using data that reflects real-world distribution, without resorting to dataset balancing" }}}\\







\textcolor{red}{\textbf{Comment R2-11 : } }
\textcolor{red}{Could the authors explain why using 90\% of the population and 30\% of a users’ data enhances robustness? Why not draw a random sample of training and testing users, as commonly done in out of bag bootstrap? Has this 90/30 approach been done before? See:}

\textcolor{red}{1. Sebastian Raschka. Model Evaluation, Model Selection, and Algorithm Selection in Machine Learning. }\\

% \cite{Raschka_2020}

% [ justify with past work ]
% 90% bc we need more data in training
% We selected random users for training
% Check the method 
% To get different sets for different iterations


We thank the reviewer for suggesting this paper. \\

First, the Population-Level Model (PLM) utilized the commonly used leave-one-out strategy, where each user's data in turn was treated as the test set, and the remaining data formed the training set. This method is particularly effective for assessing the model's ability to generalize across different users within a dataset. By randomly selecting 90\% of the remaining data for training, we introduced variability in each iteration, which is crucial for avoiding overfitting to specific data patterns and ensuring the model’s robustness. This randomness mimics real-world scenarios where models are often exposed to varied data samples, enhancing the external validity of our findings.\\

In the Hybrid Model (HM), the user's data was removed from the primary dataset to ensure that the model does not merely memorize specific user patterns but rather learns to generalize across different users. By adding 70\% of the chosen user's data to the training set, we aimed to introduce a degree of personalization, hypothesizing that incorporating some user-specific data would enhance model accuracy. While the split should depend on the problem at hand, and the amount of data available for training, the 70\%-30\% split is commonly used in machine learning \cite{joseph2022optimal, nguyen2021influence}, striking a balance between having enough data for robust training and a sufficient amount for unbiased testing.\\

Finally, the Community-Based Model (CBM) follows a similar approach but extends it to include data from a user-defined community. This method acknowledges the social and environmental factors that might influence user behavior and mood. By randomly sampling 90\% of community data, we aimed to capture a diverse set of behaviors and patterns, enhancing the model's ability to generalize across different community dynamics.\\

In all three models, using 90\% of the population/community data for each iteration was a deliberate choice to simulate a realistic distribution of training data, akin to what a model would encounter in a practical application. This method helps in understanding the model's performance in diverse scenarios and ensures the development of more robust and generalizable models. Additionally, the 70\%-30\% user data split is not only a standard practice but also provides a good balance for learning personalized patterns without risking overfitting.
\\

In response to this review, we clarified these points in the paper.\\

%\lakmal{[DONE WAGEESHA: may be add a sentence or two summarizing this to the paper, and mention that we clarified it in the paper. YOu can use text from the content I wrote above. ]}


\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 4 p.11 -> "In the above approaches, we used random sampling of 90\% of data in order to capture the diverse behavior of users, ensuring model generalization. Additionally, the 70\%-30\% user data split is standard practice and provides a good balance for learning personalized patterns without risking overfitting.}" }}\\



%\lakmal{\textbf{[DONE WAGEESHA: response to the second point about 70-30 is not clear. Did we do 90-30 splits somewhere? Be more descriptive of what you used, and clearly provide. Do not use our own prior work as references to justify techniques.]}}
% Second, many of the past works have used the 70\% 30\% split of data when training and testing the models \cite{Meegahapola2021OneMoreBite, Bangamuarachchi2022Sensing, KarimAssi2023}.  \\

% \cite{muller2022analysis} - 60% as training . 
% \cite{xu2018splitting} - random sampling method , 50- 70 % training  - et a good model


% Furthermore, multiple studies used the same approaches to use different percentages of data when training the models. For example, Kao et al.  \cite{kao2020user} used random sampling 

% \textit{\textcolor{gray}{Concrete Changes :}}\\
% {\small\textit{\textcolor{gray}{Introduction p.03 -> "" }}}\\
%\wageesha{NOTE: no studies found with 90\% random sampling of population data. Only found 70\% and 60\% sampling papers}\\


\textcolor{red}{\textbf{Comment R2-12 : } }
\textcolor{red}{For the hybrid and community-based models, were users’ data split temporally between training/testing? Otherwise, models are trained with data “from the future”, and do not offer generalizable insights for a real-world deployment (eg, how much user data is needed before we can then start having a model make predictions), introducing a form of data leakage. See:}

\textcolor{red}{1. Sayash Kapoor and Arvind Narayanan. 2022. Leakage and the Reproducibility Crisis in ML-based Science. Retrieved July 15, 2022 from http://arxiv.org/abs/2207.07048.}\\



% Not connectino between diff iteration data
% Check if the user data was split randomly or just splitting  - random splitting 
%\lakmal{\textbf{[DONE WAGEESHA: the answer is not very clear to me. Be more descriptive and provide more details.]}}\\

% In both CBM and HM, the data was randomly split into training and testing. However, the testing was not included in the training set. There is a clear separation of training and testing data. Hence, we can confirm that there is no data leakage when creating these models. We decided to split data randomly to check the models' performance in multiple iterations and average the results. 

In both CBM and HM, the primary dataset was randomly split into training and testing sets. However, for the data of the selected user, 70\% was randomly chosen and added to the training set, while the model was tested with the remaining 30\% of the user's data. This was also done while ensuring no data leakage between the training and testing splits. We randomly selected 70\% of the user data to facilitate multiple iterations of model training and testing, thereby ensuring a different training and testing set in each iteration. Notably, this methodology of randomly splitting data into training and testing sets aligns with past studies. Kao et al. \cite{kao2020user} evaluated model performance by randomly sampling health labels from the primary dataset as the training set for each user across multiple iterations. Xu et al. \cite{xu2018splitting} utilized a bootstrap and Monte-Carlo cross-validation method to randomly sample data for a given dataset, iterating the process multiple times. They demonstrated that a random sampling method maintaining a reasonable balance between the training and testing sets (50\%-70\% for training) can be considered effective for modeling. We also agree that splitting based on time could also be another cross-validation approach. We will add this as the limitation of the paper. Regardless of this split, we made sure there is no data leakage between sensor data segments, as there were time gaps between 2-7 hours across the two datasets, between two data points captured from users. \\

Moreover, we agree with the notion provided in the suggested paper regarding temporal leakage. However, it is important to clarify that compared to other time series tasks, here, by the design of the studies that collected data, the primary assumption is that there is no relation between consecutive self-reports regarding eating behavior and mood, simply because they were captured at least 2-7 hours apart across MEX and MUL datasets. This assumption is the reason why inferences are not performed throughout the time series (because ground truth is not available throughout time for tasks like eating). Here are some more recent papers that used datasets that have similar characteristics to ours, that used such random samples for robustness \cite{liao2018just, mazankiewicz2020incremental, li2020extraction}. This mutual exclusive nature and the assumption is indeed provided in the original paper that presented the MEX data \cite{meegahapola2021one}: \textit{"Moreover, we prepared the base dataset (in Section 5) assuming that individual eating episodes are mutually exclusive (similar to prior studies regarding mobile app deployments in-the-wild [24, 67, 90, 103, 106]). By making this assumption, we created a general dataset for the worst-case scenario where no temporal relationship between eating events for a given individual is assumed..."}. Hence, in response to this review, we clarified this point across many sections as given below and also added some details to the limitations section. \\

%\wageesha{In both CBM and HM, the primary dataset was randomly split into training and testing. However, when splitting the data of the selected user, 70\% of the user data was randomly selected and added to the training set. The model was tested with the remaining 30\% of data. Hence, there was no data leakage between the training and testing dataset. We randomly selected 70\% of user data in order to run the model training and testing for multiple iterations. So that in each iteration, we have a different training and testing set.}

% \cite{kao2020user}  - random sampling - user based collab filtering - random sampling 5 health labels as training set and repeat 50 iterations for each participants



%\wageesha{Notably, this methodology of randomly splitting data into training and testing data aligns with past studies. Kao at al. \cite{kao2020user} evaluated the model performance by randomly sampling health labels from the primary dataset as the training set for each user in multiple iterations. Xu et al. \cite{xu2018splitting} used a bootstrap and monte-carlo cross-validation method in order to sample data randomly for a given dataset and iterate the process multiple times. Moreover, they have shown that a random sampling method with a reasonable balance between training and testing set (50\%-70\% for training) can be considered a good model. }\\

% Notably, this methodology of randomly splitting data into training and testing data aligns with past studies done in multi-modal sensing research area \cite{KarimAssi2023, Bangamuarachchi2022Sensing, meegahapola2023generalization}.  \\



\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 4 p.11 -> "When conducting experiments, for each target user, the model training was done using 70\% of that user's randomly sampled data and a randomly sampled portion of data from other users (90\%) combined. The remaining data of the target user (30\%) was used to test the model. The training set did not contain the testing data of the selected user" }}}\\


{\small\textit{\textcolor{gray}{Section 7.3 p.23 -> Another limitation might arise from how we divided individual data for the HM and CBM model types. Kapoor and Narayanan [66] highlighted the issue of temporal leakage in time series data, which is crucial to consider. Previous studies [ 76, 79, 87] have addressed ..... Therefore, while we employed random user data splits, future research should approach such decisions cautiously, considering the nature of data, study designs, and underlying assumptions} }}\\









\textcolor{red}{\textbf{Comment R2-13 : } }
\textcolor{red}{In the Community-Based Models section at the beginning of 4, what are “th” values? If this is explained later, please define this term sooner, i.e. the first time you use it.}\\


Thank you for this comment. We modified the method section to introduce the details earlier.\\ 


\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 6.1.2 p.16 -> "Threshold Selection. The similarity values calculated in the previous step were considered as threshold values,
which can be used to filter users similar to the target user." }}}\\






%-------------------------------------------------
%-------------------------------------------------
%-------------------------------------------------

\textcolor{red}{\textbf{Results}}\\

\textcolor{red}{\textbf{Comment R2-14 : } }
\textcolor{red}{I know that data collection was not a part of this study, but I would appreciate a summary table describing the datasets with demographic information. This helps readers understand how generalizable the conclusions are to other datasets or the real world.}\\


Thank you for the comment. We added dataset details to the appendix section.\\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Appendix p.35 ->  Table \ref{table:MUL_demographocs} }}}\\

{\small\textit{\textcolor{gray}{Section 3.2 p.10 -> "Additional demographic information is given in Table \ref{table:MUL_demographocs}}" }}\\




\textcolor{red}{\textbf{Comment R2-15 : } }
\textcolor{red}{Is it true that people use their phone while resting and walking, but not while Eating, Studying, and Working? It seems reasonable that individuals may take phone breaks while studying and working, and are unlikely to use their phone in some aspects of resting (eg, napping).}\\

% \begin{figure*}[t]
% \begin{center}
%     \begin{minipage}[t]{\textwidth}
%         \centering
%         \includegraphics[width=0.7\textwidth]{images/complex_activities.pdf}
%         % \caption{}
%         % \label{fig:complex_activity_bar_chart}
%     \end{minipage}
% \end{center}
% % \vspace{0.035 in}
% \end{figure*}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{images/complex_activities.png}
% \caption{Write some caption here}\label{visina8}
\end{figure}

% [ ] remove sleeping
% Eating, studying and working have reasonable datapoints - add to cover letter
% Less datapoints were collected during outdoor activities
% Explicitly asked for datapoints during eating activity

The above diagram shows the distribution of the activities performed during daily life in the MUL dataset. As shown in the diagram, users use their mobile phones during activities such as studying and eating. Moreover, fewer self-reports were collected during outdoor activities such as walking, sports, and shopping. In addition, there were few self-reported during resting activity. We are happy to include such a distribution in the paper in case the reviewer sees value in including it. \\


% \textit{\textcolor{gray}{Concrete Changes :}}\\
% {\small\textit{\textcolor{gray}{Introduction p.03 -> "" }}}\\

\textcolor{red}{\textbf{Comment R2-16: } }
\textcolor{red}{Could error bars be added to the bar and point plots in Figures 3, 5, and 6, so we understand if the reported accuracies are consistent across the different randomly sampled test sets used? It’s difficult to make any conclusions without knowing how test set variability influences model performance.}\\


% [ add sd to figures ]

Thank you for this suggestion. We added the standard deviation values to the figures.\\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Fig. 3, 5 and 6 -> Edited the figures. }}}\\




\textcolor{red}{\textbf{Comment R2-17 : } }
\textcolor{red}{In Figure 5, it appears that the community size impacts accuracy in the MEX dataset more than the MUL dataset? Does this tell us something about the needed community specificity to make models work? It’s also interesting that the accuracy in the MUL dataset is so much lower. The authors should reason through this a bit, either in the results or the discussion.}\\


% [ discuss results. Have more data for individual users in MEX  dataset ]
% Country specific data - can get more accurate results

% https://dl.acm.org/doi/abs/10.1145/3569483 - mex dataset had more results
% https://dl.acm.org/doi/10.1145/3577190.3614129 - country specific

% Dataset datacollection method is changed 
% Add to discussion and results 

% mex 51.7% pos 9.8 neg, mul 83 pos 2.2 neg

Thank you for this comment. The MUL dataset demonstrates comparatively lower accuracies, primarily for two reasons. (i) Compared to the MEX dataset (positive 51.7\%, negative 9.8\%), the MUL dataset has a more unbalanced dataset where the percentage of positive labels is 83\%, and the percentage of negative labels is 2.2\%. Hence, when building the models, this leads to more positive labels for the selected users included in the training set. (ii) The MUL dataset spans eight countries, introducing diverse user behaviors and contexts. In such situations, performance usually declines compared to country-specific performance. This has been studied in a few of our past work where country-specific models performed better than multi-country models \cite{meegahapola2023generalization, KarimAssi2023, kammoun2023understanding}. \\

We also added an additional explanation of Figure 5 to the result section. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 6.2.1 p.17 -> "The comparatively lower accuracies observed in the MUL dataset can potentially be explained by: (i) Compared to the MEX dataset.." }}}\\





\textcolor{red}{\textbf{Comment R2-18 : } }
\textcolor{red}{Figures 7, 8, and 9 are difficult to read, as the axis ticks, axis labels, and legends are small text. Please adjust. Also, I am not sure Figure 7 is as useful as putting error bars around the values in Figure 5, specifically for both the accuracy and the community size, which would give much more information. Finally, please use feature names in the y-axis of Figures 8 and 9 that help readers understand what these features are. For example, “location\_speed\_mean” would be more understandable if it was “Average Speed”.}\\

% [ edit figures ]
We modified the figures to make things more understandable.\\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Fig. 5, 7, 8, 9 -> Edited the figures }}}\\







%-------------------------------------------------
%-------------------------------------------------
%-------------------------------------------------

\textcolor{red}{\textbf{Discussion:}}\\

\textcolor{red}{\textbf{Comment R2-19 : } }
\textcolor{red}{I would appreciate some added discussion around who are the appropriate users for mood-while-eating prediction models. For example, is it appropriate to use these models in an eating disorder population? Is it possible these models create feedback loops that negatively impact a user, which worsens eating behaviors? Think about a clinician who may read this work and want to conduct a similar study. In what populations would it be appropriate/inappropriate to conduct such a study in? I worry about automated approaches in this field broadly, due to recent news, for example, of chatbots that gave poor advice to eating disorder clients. See:}

\textcolor{red}{https://www.npr.org/sections/health-shots/2023/06/08/1180838096/an-eating-disorders-chatbot-offered-dieting-advice-raising-fears-about-ai-in-hea}\\


% [ edit discussion. 
% Usage: people who uses mobile health applications on daily basis, 
% to notify the caregivers
% Impact : might trigger people with ED, 
%  ]
% Agree to comments
% Mobile health
% Detection - sensing eating
% Characterization - https://dl.acm.org/doi/10.1145/3577190.3614129 - our paper in this 
% Intervention - not matured in mobile health, we cant come to a conclusion with our results , need to address in the future studies, need many characterization related studies in order come to conclusions. 
% https://dl.acm.org/doi/abs/10.1145/3463492	- vulnerability and receptivity - 
% Under explored areas
% Add to discussion

% https://www.npr.org/sections/health-shots/2023/06/08/1180838096/an-eating-disorders-chatbot-offered-dieting-advice-raising-fears-about-ai-in-hea

We thank the reviewer for suggesting this article and agree with the given comment. There is a possibility that smartphone interventions for eating moods could trigger users with eating disorders. We have added a section in the Limitations to discuss this issue, referencing the suggested article.\\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 7.3 p.22 -> "Exploring how smartphones can provide feedback and interventions by considering the user's mood while eating has its own challenges, for example, concerning the risk of triggering individuals with eating disorders. Given the research done in the mobile health research area, providing interventions to users is still in an evolving stage. Without the maturity of this research area and the current results we have, we cannot come to the conclusion that these interventions can negatively or positively affect the users. One of the past studies discussed how crucial it is to time the delivery of the intervention to the users correctly and how the user might not be ready to process these interventions \cite{mishra2021detecting}. Another study was done regarding the National Eating Disorders Association's (NEDA) chatbot that offered dieting advice where many users with eating disorders found the advice given by the AI tool was triggering their conditions \cite{Wells_2023}. Future work should address these limitations and consider conducting comprehensive studies to provide more conclusive insights." }}}\\





==> review-old/R3.tex <==
\newpage 
\textcolor{red}{\begin{center}\textbf{Reviewer 3 }\end{center}}

\textbf{Recommendation: Reject}\\

\textcolor{red}{\textbf{Comments:}}
\textcolor{red}{The topic of mood recognition is of significant interest to ACM Health. However, I recommend rejection for this submission due to several reasons outlined below. I hope my feedback proves constructive for future submissions.}\\


\textcolor{red}{\textbf{Comment R3-1 : } }
\textcolor{red}{The paper's structure and clarity leave room for improvement. The introduction, for instance, is overly lengthy and deviates from the conventional structure, making it challenging to follow.} \\

We apologize if the structure of the paper was difficult to follow. It was not entirely clear to us from the review what specific structural changes were required. However, in the revised version, we have restructured the paper to address the comment where we believed changes would benefit the paper. The revised paper now organizes the main topics according to the research questions. Under each research question, the method and results are presented. We hope this revision will make the paper easier to follow. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{RQ1, RQ2, RQ3 sections were clearly separated, and method and results are given under each Section.}}}\\







\textcolor{red}{\textbf{Comment R3-2 : } }
\textcolor{red}{The importance of analyzing moods during eating isn't well justified. From a medical standpoint, daily mood fluctuations would likely be of greater relevance than short-term moods experienced during meals. The motivation behind the research is not sufficiently clear.}\\

% [ mood can be changed in shorter time periods and important to monitor - find past work
% Daily mood while eating hard be monitor, at end of the day people may forget about the mood of the day
% To send notifications while eating, need to monitor short-term mood
% ]
% Daily mood is important
% Medical papers - instantaneous mood and eating
% Eating - mood connectino
% Review 2  - add to intro

% \cite{macht2008emotions} - Thus, emotion-induced changes of eating can be a result of interference of eating by emotions, a by-product of emotions, and a consequence of regulatory processes (i.e., emotions may regulate eating, and eating may regulate emotions).

% This study examined the relationship between coping efforts and stress-related mood changes

% \cite{carroll2013justintime} - s primarily ate when they were stressed. emotional eating - real-time sensor data wearable sensors 

While we agree with the reviewer's perspective regarding the importance of daily mood assessment, a large body of work in computing \cite{dicerson2011empath, narziev2020stdd, can2019continuous, servia2017mobile, likamwa2013moodscope}, psychology \cite{gardner2014better, dubad2021clinical, malhi2017promise}, and nutrition science \cite{polak2015measuring, bisogni2007dimensions, jastran2009eating} highlights the importance of continuous mood and stress monitoring. One study demonstrated that changes in eating behavior can result from the current mood, and conversely, mood can influence eating behavior \cite{macht2008emotions}. Additionally, another study underscored the significance of continuous mood monitoring to capture emotional eating using wearable sensors \cite{carroll2013justintime}. Tracking daily mood during meals can be challenging, as users may forget their emotional states by the end of the day. Therefore, it is necessary to send notifications around meal times to capture short-term mood changes. In response to the R2-2 comment, we have revised the introduction section to emphasize the importance of understanding mood during meals. We hope these changes adequately address this review. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Introduction p.02 -> "Mental well-being and eating behavior have been the subjects of numerous studies, both individually and in conjunction with each other..." }}}\\









\textcolor{red}{\textbf{Comment R3-3 : } }
\textcolor{red}{The paper also lacks depth and insight. For instance, it does not adequately differentiate between moods experienced while eating versus during other activities. The distinction between these states and the reasons for focusing specifically on eating are not clearly articulated.}\\

% [ discussion on mhealth apps, dietary monitoring apps usage 
% ]
% Length paper
% Only can use one dataset 
% Already studing for diff context and mood in another study with country differences - large scope
% Will not be disccsussed n this paper
% Discuss why mood is important while eating

Thank you for this comment. First, while we have two datasets, we can only study mood during other activities using the MUL dataset \cite{meegahapola2023generalization}. This limitation exists because, during the collection of the MEX dataset \cite{Meegahapola2021OneMoreBite}, mood data was gathered solely during eating activities. Therefore, we do not have mood reports for other activities. Additionally, the focus of this paper is not on mood during other activities. Studies have already been conducted using the MUL dataset to explore mood during various activities and to infer general mood \cite{morshed2022food, kammoun2023understanding, meegahapola2023generalization}. For instance, one study aimed to infer general mood \cite{meegahapola2023generalization}. Furthermore, other research has been carried out to infer moods in different contexts \cite{zepf2020driver, zhu2015naturalistic, scott2006effects, katsis2008towardemaotion, burns2011harnessing} and to examine how moods vary based on location in different countries \cite{meegahapola2023generalization}. Moreover, another paper published at ACM HEALTH emphasized the need to understand the interconnection between food, mood, and context \cite{morshed2022food}. Therefore, while we would have liked to include a broader discussion around mood during other activities, we will not discuss these aspects in this paper, due to page limitations and the focus of the paper. However, as a response to this review, we will add to the discussion section that studying mood during other activities in more depth could be an interesting direction to look into. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 7.3 p.22 -> "In this study, we explore the mood while eating. However, it is worth exploring the mood in other contexts as one study emphasized the importance of understanding the food, mood, and context \cite{morshed2022food}. Hence, future studies could focus on studying mood during other activities." }}}\\






\textcolor{red}{\textbf{Comment R3-4 : }}
\textcolor{red}{Technically, the paper does not present any unique challenges or solutions. The issues of data scarcity and domain transfer problems are well-documented in classification tasks, and there's a wealth of existing research addressing these problems. It would be beneficial to identify and address unique technical challenges within this specific context.}\\

% Sub population shift not studied for mobile health area - only resently studues done in this area
% Domain transfer problem - mobile Sensing  data area  multimodal setting,,  mood inference (unique situated context ) not very discussed, 
% CV, NLP, speech have discussed these
% https://dl.acm.org/doi/abs/10.1145/3380985 - domain adaptation techniques - not work for mobile sensing area, 

Most domain transfer and generalization-related problems have been extensively studied in other research areas such as computer vision \cite{sankaranarayanan2018learning, zhang2016lsdt} and NLP \cite{ramponi2020neural}. Only recently have studies begun to address the domain shift and generalization problem in mobile sensing \cite{xu2023globem, meegahapola2023generalization}. Our group has been exploring this direction for some time within the context of the larger European project, WeNet. Furthermore, previous work in mobile sensing indicates that techniques used in computer vision and natural language processing cannot be directly applied to mobile sensor data due to numerous nuanced differences across data modalities \cite{chang2020systematic}. Here are some papers discussing the distinctions between different research domains and outlining drawbacks in mobile sensing data, including future directions \cite{merrill2023self, chang2020systematic, merrill2023homekit2020, xu2023globem}. These papers are directly from researchers working in the sensing domain. Therefore, we do not concur with the reviewer's view that a significant amount of prior work has explored domain transfer and generalization issues. We strongly believe that problem areas explored in other data modalities should still be investigated in the context of mobile sensor data. Additionally, mood inference in a specific context has not been discussed extensively in this research area.\\

% \cite{chang2020systematic} - We observe that the HAR model has an F1 score of 0.94 when it is tested on the same body position on which it was trained (
% However, in the presence of domain shift, the F1 score of the classifier drastically reduces to as low as 0.05 when the model is tested on IMU data from the forearm
% we study the problem
% of wearing diversity which pertains to the placement of the wearable sensor on the human body, and demonstrate that even state-of-the-art deep learning models are not robust against these factors.


Furthermore, in previous work by Chang et al. \cite{chang2020systematic}, the issue of domain shift was discussed, highlighting the challenges faced when domain adaptation techniques are applied to mobile sensing areas, emphasizing the need to examine models and architectures used in other domains for mobile sensor data. \\

% \textit{\textcolor{gray}{Concrete Changes :}}\\
% {\small\textit{\textcolor{gray}{Introduction p.03 -> "" }}}\\







\textcolor{red}{\textbf{Comment R3-5 : } }
\textcolor{red}{The explanation of experiments and results is another area that needs improvement. The reasons behind regrouping five mood classes into three are not explicitly stated.}\\

% Justify with past studies

We thank the reviewer for pointing this out. As a response, we have improved the explanation regarding regrouping the five mood classes into three. This decision was motivated by prior work in mental health and sensing \cite{meegahapola2023generalization}. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\

{\small\textit{\textcolor{gray}{Section 2.1 p.05 -> "As such, throughout this study, we consider these three levels as a fundamental construct in relation to self-reported mood-while-eating, in line with previous studies \cite{wampfler2022affective, soleymani2011multimodal, meegahapola2023generalization, kammoun2023understanding}." }}}\\








\textcolor{red}{\textbf{Comment R3-6 : } }
\textcolor{red}{There's a lack of detailed analysis regarding which features contribute to mood based on the results. For example, do the results indicate that watching YouTube while eating results in a bad mood? This type of interpretation could provide readers with practical insights. }\\

% [ not enough space to add a descriptive analysis ]
% Feature impotence - modify


% At the initial stage of the paper, we included the statistical and descriptive analysis for the datasets. However, with the page constraint, the sections with those analyses are removed from the paper. \\ 

% feature importance - improve
% cannot claim 
% 

Thank you for this comment. In response, we have expanded the discussion on feature importance in Section 6.2.3. Due to the way in which the two datasets have been collected and with the current inferences, we cannot causally assert which features directly affect a user's mood in practical situations, as our study only provides analytical findings based on correlations. \\


\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 6.2.3 p.19 -> " In this section, we explore the Gini feature importance for mood inference, generated using Random Forest classifiers for CBM with passive sensing features, using both MEX and MUL datasets..." }}}\\








\textcolor{red}{\textbf{Comment R3-7 : } }
\textcolor{red}{Additionally, the reason for the low accuracy, especially as displayed in Figure 3, needs to be addressed.}\\

% Plm model results are usually lower - > that why we purpose this new method

% https://dl.acm.org/doi/10.1145/3569485 - depression inference lower results for plm

% https://dl.acm.org/doi/abs/10.1145/3596246 - Stress inference lower results - discussion

% https://dl.acm.org/doi/abs/10.1145/3569483 - mood inference 

The results depicted in Figure 2 (previously Figure 3 before reformatting the paper) represent the outcomes of the population-level models using the MUL dataset. Commonly, results from population-level models tend to be lower. For instance, past studies have shown that inferences on depression \cite{xu2023globem}, stress \cite{yu2023semi}, and general mood \cite{meegahapola2023generalization} using baseline methods, such as population-level models, do not yield high performance. The rationale behind proposing a new personalized model in our study is to enhance the results obtained for mood inference with the population-level models. \\

% \textit{\textcolor{gray}{Concrete Changes :}}\\
% {\small\textit{\textcolor{gray}{Introduction p.03 -> "" }}}\\










\textcolor{red}{\textbf{Comment R3-8 : } }
\textcolor{red}{Finally, I highly recommend a thorough revision of the paper for improved readability and comprehension. The current structure and style make it difficult for the reader to follow and comprehend the content.}\\


Thank you for providing feedback on the structure of the paper. As mentioned in our response to R3-1, we have modified the structure of the paper in areas where we believed improvements were needed. In addition, we re-wrote many sections of the paper, to make it more coherent and readable. We hope that our revisions will be sufficient.\\



% \textit{\textcolor{gray}{Concrete Changes :}}\\
% {\small\textit{\textcolor{gray}{Introduction p.03 -> "" }}}\\







==> review/00-responses.tex <==
\textcolor{black}{\begin{center}\textbf{Reviews and Responses}\end{center}} 

We thank the reviewers for their valuable comments that were helpful in reshaping the paper. In this document, we have listed all the review comments and our responses, including the changes that were made. To facilitate reading, we use \textcolor{red}{\textbf{red}} color to indicate the original comments, \textcolor{black}{\textbf{black}} color to provide our responses, and \textcolor{gray}{\textbf{gray}} color to indicate the concrete changes made to the paper.


\input{review/R0-summary}
\input{review/R1}
\input{review/R2}
\input{review/R3}

\newpage

==> review/R0-summary.tex <==
\textcolor{red}{\begin{center}\textbf{Summary meta-review}\end{center}}

\textbf{Recommendation: Major Revision}\\

\textcolor{red}{Below, I have summarized the major concerns along with revision suggestions. Please carefully review the reviewers' detailed comments as well and ensure that all points are addressed in the next revision.}\\


\textcolor{red}{1. Provide a clear explanation of how the test dataset is downsampled, and rerun the experiments using an unmodified test set if feasible. Demonstrate that the results are generalizable to real-world scenarios.}\\

We have re-done the experiments with the unmodified testing sets, without any downsampling. Please refer to the response to Comment R2-3. Moreover, we have added the 5-class model performances to the paper's appendix. Please refer to the response to Comment R3-5.\\


 
\textcolor{red}{2. The stated contributions should be scaled back due to inconsistencies in the test sets across models.}\\

We changed the tone of the wording, and removed all the strong comparisons of models. Please refer to the responses to R2-3 and R3-5 for more details.\\



\textcolor{red}{3. Justify the motivation behind the study and its feasibility.}\\

We added more details to justify the motivation. Please refer to the responses R3-1 and R3-2 for more details. \\



\textcolor{red}{4. Provide a clearer explanation of the paper's technical contributions in comparison to the state-of-the-art work, and explain how the experimental results support these contributions.}\\

Please refer to the response to R3-4.\\









==> review/R1.tex <==
\newpage 
\textcolor{red}{\begin{center}\textbf{Reviewer 1 }\end{center}}

\textbf{Recommendation: Accept}\\

\textcolor{red}{\textbf{Comments:}}\\
(There are no comments.)


==> review/R2.tex <==
\newpage 
\textcolor{red}{\begin{center}\textbf{Reviewer 2 }\end{center}}

% \textit{\textcolor{gray}{Concrete Changes :}}\\
% {\small\textit{\textcolor{gray}{Section 2.5, p.08 -> ""}}}\\

\textbf{Recommendation: Major Revision}\\


\textcolor{red}{\textbf{Comments:}}\\

\textcolor{red}{Thanks for responding to my comments. I appreciate the clarification on the Mexico/multi-country studies, random sampling across all model types, and the added discussion on implementation.}

\textcolor{red}{I still have a few comments that I believe need to be addressed before I can recommend this paper for minor revisions or publication. My remaining major concerns are that (1) the contributions need to be scaled back due to the misaligned test sets across models. More importantly, I am worried that (2) the results are not generalizable to the real world if the test set was downsampled.}\\

\textcolor{red}{\textbf{Possible improvements:}}\\


\textcolor{red}{\textbf{Comment R2-1 : } }
\textcolor{red}{Maybe include in the abstract not just “two separate datasets” but “two separate datasets from two separate studies”? It gives a bit more information to infer that the data cannot be combined.}\\

Thanks for bringing up this valuable point. We mentioned this in the abstract and contributions.\\ 

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section Abstract, p.01 -> "we analyzed everyday eating behavior and mood using two separate datasets from two different studies:"}}}\\


\textcolor{red}{\textbf{Comment R2-2 : } }
\textcolor{red}{I agree that the test sets cannot be aligned and appreciate the added limitation (“...fair comparison of the results …”). I do believe it is still misleading to make statements such as “hybrid models … can perform better than population-level models” since adequate comparison cannot be made across these model types. I recommend removing all comparators across model types and reframing the contribution. For example, you could simply state “hybrid models achieved x\% accuracy for Mexico and y\% accuracy for the multi-country dataset.” Similar revisions should be made across the entire manuscript in all statements to remove direct comparators (eg, “better”, “worse”) when comparing model results.}\\

We agree. As a response to this comment, we went through the whole manuscript, and removed such direct comparisons. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 1, p.04}}}\\
{\small\textit{\textcolor{gray}{Section 6, p.17}}}\\
{\small\textit{\textcolor{gray}{Section 7, p.20}}} \\



\textcolor{red}{\textbf{Comment R2-3 : } }
\textcolor{red}{Thanks for clarifying that SMOTE was not used on the testing set. I’m still a bit confused about what is meant when the manuscript states “For testing sets, we down-sampled majority classes.” Shouldn’t the test set class balance not be adjusted at all, otherwise the results are not generalizable to the real world, since the test set does not reflect the real world distribution? I believe if the class balance was adjusted to the testing set, the experiments need to be rerun without class balancing in the test set. See recommended steps in the following paper, where the test set is not manipulated at all, and only reports model performance:}

\textcolor{red}{[1] Raschka S. Model Evaluation, Model Selection, and Algorithm Selection in Machine Learning.}

\textcolor{red}{Not academic, but searches show from data science blogs/posts why adjusting the test set in is not good practice. See:}

\textcolor{red}{https://stackoverflow.com/questions/55921286/should-i-balance-the-test-set-when-i-have-highly-unbalanced-data
https://www.analyticsvidhya.com/blog/2017/03/imbalanced-data-classification/
https://datascience.stackexchange.com/questions/17873/imbalanced-dataset-how-to-deal-with-test-data}\\

% imbalanced testing results w accuracy, auc-roc and f1

Thank you for the insightful comment. To address your concern, we have revised the manuscript to include results from testing on an imbalanced dataset, as recommended. Results under RQ1 were already following this approach. These updated results were derived by training and evaluating the models without altering the test dataset, ensuring that the class distribution reflects real-world conditions. Additionally, we have expanded the performance metrics to include AUC-ROC values alongside accuracy and F1 scores, providing a more comprehensive evaluation of the model's performance. We believe these changes enhance the robustness and clarity of our findings. \\


\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 4, p.11 -> "SMOTE was applied to the training set to obtain an upsampled dataset. The testing set remained unaltered to reflect real-world scenarios, where oversampling and undersampling are not performed during inference."}}}\\
{\small\textit{\textcolor{gray}{Section 5.2, p.14 -> Table 2}}}\\ 
{\small\textit{\textcolor{gray}{Section 6.2, p.17, p18 -> Fig 5, Fig 6}}}\\




\textcolor{red}{\textbf{Comment R2-4 : } }
\textcolor{red}{Thanks for providing assumptions and papers regarding the claim that your splitting approach is valid for hybrid models and we cannot assume that temporal leakage has occurred. I still do not agree with the approach, as I believe we should always try to simulate the real world and in this case the logical thing would be to split the training/testing for personalized models at some specific temporal point for each participant. In a real life deployment, we would never have access to future information to train machine learning models.}
\textcolor{red}{That said, I don't have a concrete example to justify why this might prove problematic given the specific features and outcomes used in the paper, so I think my comment has been addressed enough with the limitation. I would consider splitting temporally in future “personalized model” approaches you use.}\\

We thank the reviewer for their thoughtful comment and valuable feedback regarding the personalized models. We agree that simulating real-world scenarios is essential. In future work, we will carefully consider temporal splitting for personalized models to ensure the approach aligns with real-world scenarios. \\  





\textcolor{red}{\textbf{Comment R2-5 : } }
\textcolor{red}{ I’d recommend adding to 6.1.2 “considered as threshold (th) values”, so that the acronym is clearly defined.}\\

Thank you for this comment. We made this change in the manuscript.\\ 

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 6.1.2, p.16 -> " considered as threshold (th) values"}}}\\




\textcolor{red}{\textbf{Comment R2-6 : } }
\textcolor{red}{Thanks for the figure on smartphone use during specific activities. I’d recommend putting the figure in the appendix so that this assumption is validated.}\\

Thank you for the comment. We added the figure to the appendix.\\


\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 4, p.12 -> "(see Figure 11)"}}}\\
{\small\textit{\textcolor{gray}{Appendix, p.32 -> "Fig. 11"}}}\\



\textcolor{red}{\textbf{Comment R2-7 : } }
\textcolor{red}{Thanks for providing the standard deviations in the Figures. Pretending we disregard my prior point on misaligned tests, I think these standard deviations actually verify we cannot claim, even empirically, that hybrid models are better than population level models (contribution 2). This is because for the MUL dataset, the accuracy of the population model (43.6) falls within one standard deviation of the hybrid model accuracy (mean 50.3, standard deviation 20.6). You could adjust the contribution to state that hybrid models were better for the MEX dataset, but not the MUL dataset. That being said, because of my comment on misaligned datasets, I do not think we can say that hybrid models or community models are “better”.}\\

As a response to the previous comment (R2-2), we removed such comparisons throughout the paper. Hence, this issue will not be present in the new manuscript. \\

\textcolor{red}{\textbf{Comment R2-8 : } }
\textcolor{red}{I’d also recommend drawing actual error bars showing the standard deviations instead of or in addition to writing the standard deviation, so that these overlaps are clearer.
Please add error bars (eg, standard deviations) to Figure 6, F1 scores as well, so we understand the distribution of F1 scores across test sets, and if one model is actually better than the other in terms of F1 score.}\\

Thank you for the comment. We have added the error bars to the figures. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 6.2, p.18 -> Fig 6}}}\\



==> review/R3.tex <==
\newpage 
\textcolor{red}{\begin{center}\textbf{Reviewer 3}\end{center}}

\textbf{Recommendation: Reject}\\

\textcolor{red}{\textbf{Comments:}}

\textcolor{red}{I strongly recommend rejecting this paper due to its failure to address my concerns adequately.}\\

\textcolor{red}{\textbf{Possible improvements:}}\\


% ================================================================================
% ================================================================================
% ================================================================================

\textcolor{red}{\textbf{Motivation and Feasibility}}\\

\textcolor{red}{\textbf{Comment R3-1 : } }

\textcolor{red}{While the paper underscores the significance of mood recognition, a widely acknowledged point that requires minimal elaboration, it falls short in justifying why studying mood recognition during eating is important. }\\

We thank the reviewer for their insightful comment and we agree with the importance of further justifying the value in identifying mood recognition with eating episodes. Many studies have shown that dietary behaviors significantly influence mood, and vice versa. For instance, fasting and low card diets have been shown to improve mood, supporting therapy for chronic pain syndromes in the long term \cite{westman2002effect, Michalsen2010, Fond2013}. Additionally, some studies have shown that eating habits reduce tension, anger, confusion, and overall mood while improving positive mood \cite{Hussin2013}. The connection between gut health and brain function also shows the importance of eating habits, as past research indicates that gut health directly impacts cognitive abilities and mental well-being \cite{Moulton2019}. Moreover, past clinical and preclinical research further shows how dietary patterns influence anxiety, stress, and depression \cite{Luqman2024}. While anxiety and depression are separate conditions from mood, prior work has shown the value of understanding mood trajectories to reason such conditions \cite{meegahapola2023generalization}. This shows the connection between mental well-being and eating behaviors. Moreover, we would like to point to Bisogni's framework \cite{bisogni2007dimensions} regarding eating and drinking events, where mental processes are one of the main components (See Section~\ref{subsec:eating_as_a_holistic}). With all these changes, we added a modified paragraph to the introduction to justify why studying mood during eating is important. \\


\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 1, p.2 -> "Mental well-being and eating behavior have been extensively studied, both as individual phenomena and in their [...] of mood and eating data is crucial for advancing personalized health interventions and improving both individual and population-level health outcomes."}}}\\



\textcolor{red}{\textbf{Comment R3-2 : } }

\textcolor{red}{Furthermore, it neglects to establish the connection between real-time eating behavior and mood changes. Long-term changes in eating behavior are commonly associated with mood shifts; for instance, a sudden alteration in food intake may indicate depression. However, the paper focuses on mood recognition based on real-time and short-term eating behavior without providing a theoretical foundation. Without such an explanation, it is challenging to accept the premise that short-term eating behavior is linked to mood, given its inherently random nature. }


We appreciate the reviewer’s insightful comment and agree that establishing a theoretical connection between (real-time) eating episodes and mood (as well as other mental well-being constructs) is crucial for reinforcing the paper’s premise. Section~\ref{subsec:eating_as_a_holistic} extensively discusses this connection using Bisogni's holistic eating framework \cite{bisogni2007dimensions}. Rooted in nutrition science research, this framework emphasizes the importance of understanding various aspects surrounding eating episodes. Eating episodes are defined across eight dimensions, including food/drink type and amount, time, location, social setting, concurrent activities, mental processes, physical condition, and recurrence. Additionally, we have introduced a new Section 2.2 to provide further theoretical grounding. \\

Moreover, as a response to this review, we have mentioned the following aspects in the introduction and related work of the paper, from several dimensions:\\ 
\textbf{Theoretical Basis for Short-Term Eating Behavior and Mood}:
Short-term eating behavior is not inherently random but is influenced by situational and emotional factors. For example, emotional eating theory suggests that individuals often consume food in response to immediate emotional states rather than long-term dietary goals~\cite{gibson2006emotional}. This includes impulsive eating patterns triggered by stress, sadness, or happiness, which are indicative of mood changes.

\textbf{Real-Time Mood and Eating Behavior}: Research in mobile health applications has shown that real-time passive sensing can effectively capture meaningful associations between short-term eating behavior and mood. For instance, snack consumption often increases during periods of negative mood, while regular meal patterns are linked to positive emotional stability~\cite{meegahapola2021one, nahum2018just}. These findings suggest that short-term eating behaviors, such as snacking or irregular meal patterns, serve as valuable indicators of mood dynamics. Recognizing mood during eating episodes in real-time is particularly valuable for mobile health applications that deliver personalized interventions. For example, identifying emotional triggers for eating in real-time can help mitigate episodes of emotional eating, which are significant contributors to long-term health issues like obesity and depression~\cite{ha2023role}. This highlights the potential of such approaches to advance personalized health and well-being solutions.

\textbf{Contextualizing Short-Term Eating Episodes:} In the paper, we focus on mood recognition during eating events to demonstrate the feasibility of identifying mood from real-time eating behaviors. While this does not encompass the broader perspective of long-term dietary changes, it aligns with research on ecological momentary assessment (EMA), which highlights the importance of capturing real-time data for immediate emotional and behavioral states \cite{gatica2019discovering, Biel2018}. Real-time mood tracking during eating has the potential to inform timely interventions, particularly for individuals prone to emotional eating.
\\

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 1, p.2}}}\\
{\small\textit{\textcolor{gray}{Section 2.2, p.5}}}\\
{\small\textit{\textcolor{gray}{Section 2.5, p.7}}}\\



\textcolor{red}{\textbf{Comment R3-3 : } } 

\textcolor{red}{The reported accuracy of 46\% in a three-class classification is notably low and closely resembles random guessing (33.3\%). This meager improvement (46\% vs. 33\%) could potentially be attributed to overfitting during training.} \\

We can confirm that overfitting is not an issue in this case, as the model's performance on the training set is only marginally higher than its performance on the testing set. This alignment between training and testing performance was consistently monitored during model development, as routine. The modest performance reflects the inherent difficulty of the task rather than overfitting. Mood inference is a well-documented challenge in sensing research due to the noisy and complex nature of behavioral and physiological data~\cite{likamwa2013moodscope, servia2017mobile, meegahapola2023generalization, xu2023globem}. Personalization has been proposed as one of the promising solutions \cite{han2024systematic, meegahapola2023generalization}. Hence, the seemingly low accuracy is consistent with prior studies tackling similarly complex tasks, indicating that even marginal improvements over random guessing represent meaningful progress in this domain.\\




% ================================================================================
% ================================================================================
% ================================================================================

\textcolor{red}{\textbf{Method Contribution}}\\

\textcolor{red}{\textbf{Comment R3-4: } }

\textcolor{red}{The paper falls short in articulating a distinctive contribution in technical methods: domain transfer and generalization-related challenges. While the revised version references a paper acknowledging distinctions between these problems in computer vision (CV) and natural language processing (NLP) domains compared to the mobile sensing area, it fails to elucidate the specific disparities or highlight the unique challenges inherent to mobile sensing.
To enhance the paper's clarity and contribution, it is crucial to expound on the dissimilarities encountered in the mobile sensing domain in contrast to CV and NLP. The revised manuscript should explicitly outline the distinctive problems and subsequently provide a clear exposition of the novel solution proposed to address these unique challenges. Without this elucidation, the paper lacks a concrete demonstration of its methodological contribution.}\\

Thank you for this valuable comment. We agree that domain generalization and adaptation are critical challenges. In our previous work~\cite{meegahapola2023generalization, meegahapola2024m3bat}, we explored these aspects in depth and continue to focus on them in our ongoing research. Other researchers have also looked into these problems in the context of mobile sensing \cite{xu2023globem}. We would like to reiterate that model personalization under class imbalance is the key challenge we aim to address with our approach. In response to this review comment, we have revised the introduction section to emphasize this point. Additionally, the related work section (Section 2.6) is also there to clearly demonstrate how this paper fits within the context of prior research. \\

\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Section 1, p.3 -> "Finally, in terms of machine learning-based modeling, the traditional [...] are robust to user heterogeneity and a lack of sufficient data remains a challenge"}}}\\
{\small\textit{\textcolor{gray}{Section 2.6, p.8 -> "Smartphone Sensing Inference Personalization"}}}\\




% ================================================================================
% ================================================================================
% ================================================================================


\textcolor{red}{\textbf{Results}}\\

\textcolor{red}{\textbf{Comment R3-5 : } }

\textcolor{red}{The dataset employed in this study comprises five classes. Even though the primary goal is to recognize three specific emotions in this paper, it remains pertinent to report the accuracy across all five classes. Given my reservations regarding the feasibility of this work, I am inclined to question whether the accuracy for the entire set of five classes might be insufficient to substantiate the paper's claims. Therefore, presenting the accuracy for all five classes would provide a more comprehensive understanding of the model's performance and address potential concerns about its overall efficacy.}\\

Thank you for your insightful comment. We recognize the importance of presenting results for all five classes and addressing concerns regarding overall performance. In response, we have revised the manuscript to include performance (accuracy, F1-score, and AUC-ROC) for the 5-class inference task. These results have been added to the Appendix. We would also like to note that prior mobile sensing research has rarely explored 5-class inferences for mental well-being. Most studies have focused on 2-class or 3-class inferences~\cite{likamwa2013moodscope, servia2017mobile, xu2023globem, soleymani2011multimodal, meegahapola2023generalization, morshed2022food, han2024systematic, wampfler2022affective, horlings2008emotion, zhang2020corrnet}. This trend stems from findings in clinical research, which suggest that distinctions between categories such as "positive" vs. "very positive" or "negative" vs. "very negative" are not particularly useful for designing interventions. We have elaborated on this point in Section~\ref{subsec:eatingepisode}.\\

%In the MEX dataset, while the PLM model achieved an accuracy of 14.3\% and AUC-ROC of 0.47, the HM model had performance of 46.4 accuracy and 0.51 AUC-ROC. Similarly, for the MUL dataset, the HM model showed an improvement from 13\% to 62.6\% accuracy compared to the PLM. However, the results demonstrate that the 5-class classification remains more challenging than the corresponding 3-class models. \\
 


\textit{\textcolor{gray}{Concrete Changes :}}\\
{\small\textit{\textcolor{gray}{Appendix Section~\ref{sec:appendix_5-class} p.31 -> "The results presented in Table 6 summarize the mean accuracy, F1-score, and AUC-ROC values for 5-class
inference using Random Forest models on both PLM and HM..."}}}\\
{\small\textit{\textcolor{gray}{Appendix, p.33 -> Table~\ref{tab:5_class_inference_results_plm_hm}}}}\\
{\small\textit{\textcolor{gray}{Appendix, p.34 -> Figure~\ref{fig:5_class_clm_threshold_vs_acc}}}}\\

